Targeted Retrieval, Compact Representations: How CoT Reasoning Improves Long-Context Counting

Large language models (LLMs) have been rapidly improving in long-context tasks, powered by Chain-of-Thought (CoT) reasoning. However, the internal mechanisms underlying this improvement remain unclear. We investigate these mechanisms through a needle-in-a-haystack (NIAH) counting task, where an LLM is asked to count the number of records dispersed in a long text. Across twelve model comparison groups, Thinking (or reasoning) improves counting accuracy over Non-thinking, with pronounced gains at larger counts. This motivates our mechanistic analysis, which identifies two contrasting mechanisms: (i) broad retrieval, where Non-thinking models broadly attend to multiple needles; (ii) targeted retrieval, where Thinking models use enumeration in CoT traces to successively retrieve needles. Targeted retrieval concentrates attention on individual needles and is accompanied by more compact internal representations. Moreover, causal intervention analysis suggests that Thinking models use the CoT trace to maintain and update an internal counter as needles are successively retrieved, even without explicit numbering. In small controlled experiments, both retrieval mechanisms and counter states emerge under standard autoregressive training. Together, our results connect long-context retrieval with representation geometry of counting, supporting a state-tracking account of CoT reasoning.

==> environments/synthetic-quote.tex <==
%%%%%%%%%% Failed to squeeze into one line %%%%%%%%%%%%
%\vspace{0.5\baselineskip} % Adds a little space above, like a quote would
%{
%\setlength{\leftskip}{0pt}
%\small
%\noindent
%\texttt{<CountChar> T b n <S>}
%\ldots\ \textbf{T}o \textbf{b}e, \ldots\
%or \textbf{n}ot to \textbf{b}e.\ \ldots
%\texttt{<Think> <S> \textbf{T} <S> \textbf{b}
%<S> \textbf{n} <S> \textbf{b} </Think> <Ans> <4>}
%}
%\vspace{0.5\baselineskip} % Adds a little space below


\begin{quote}
\small
\setlength{\parskip}{3pt}
\noindent
\texttt{<CountChar> T b n <Sep>}
\ldots\ \textbf{T}o \textbf{b}e, \ldots\
or \textbf{n}ot to \textbf{b}e.\ \ldots
\par\noindent
\texttt{<Think> <Sep> \textbf{T} <Sep> \textbf{b}
<Sep> \textbf{n} <Sep> \textbf{b} </Think> <Ans> <4>}
\end{quote}

==> environments/table-comparison-v1.tex <==
Targeted Retrieval, Compact Representations:
How CoT Reasoning Improves Long-Context Counting
Liang Twist Shan1 Tianyu Hu2 Hao Yan1 Yiqiao Zhong1,2
1Department of Statistics, University of Wisconsin-Madison
2Department of Computer Sciences, University of Wisconsin-Madison
September 14, 2026
Abstract
Large language models (LLMs) have been rapidly improving in long-context tasks, powered
by chain-of-thought (CoT) reasoning. However, the internal mechanism of long-context infer-
ence remains unclear. In this paper, we focus on a needle-in-a-haystack (NIAH) counting case
study, where an LLM is asked to count the number of records inserted in a long text. We
found that thinking (or reasoning) consistently improves accuracy by a large margin, especially
at large counts. Further, our mechanism-level analysis shows contrasting behavior between
the two modes: (i) broad retrieval, where Non-thinking models retrieve needles with noisy
broad attention; (ii) targeted retrieval, where Thinking models retrieve needles one-by-one in
its CoT trace. Targeted retrieval shows a localized attention pattern that targets at a single
needle, accompanied by increased compactness of internal representations. Moreover, causal in-
tervention analysis suggests that models use the CoT trace to maintain and update an internal
counter as needles are targeted and retrieved, even without explicit numbering. In addition, this
count-tracking mechanism emerges under standard autoregressive training in a small controlled
experiments.
1 Introduction
Long-context reasoning has become a pillar of large language models (LLMs) in solving complex
tasks, where models generate a sequence of chain-of-thought (CoT) tokens before reaching a final
answer. Yet, existing interpretability research mostly focuses on short input prompts and model
generation includes no long CoT traces. A critical gap exists between the ever-growing inference-
time scaling and our limited understanding of model’s internal mechanism.
To understand long-context inference and CoT reasoning, we present a case study on long-
context counting partly based on needle-in-a-haystack (NIAH) benchmarks (Kamradt, 2023; Hsieh
et al., 2024). In a nutshell, this task asks the model to count the number of records (or needles,
denoted by N1, N2, N3, . . .) inserted in a long passage (haystack). For example, the following input
prompt contains two audit records followed by a query:
“<passage> . . . In the 2024 city score audit, Paris received a score of 92. . . . In the 2024 city score audit,
Vienna received a score of 73. . . . </passage>
How many city-score audit records are in the passage?”
We evaluate two types of models (or modes). A Non-thinking model typically emits a final-
answer count such as “Total: 8”, while a Thinking model generates a CoT trace enclosed in the
1
A Non-thinking: broad retrieval
Prompt
span ��1 ��2 ��3 ��10⋯ ⋯ ⋯ ⋯ ⋯
Direct
answer <Ans> Total: 8
Attention from <ans> token to needle span
N1 N2 N3
N4
N5 N6 N7
N8
N9
N10
0 Prompt position 10k tokens
Attention mass 0 0.025 ≥0.099
B Thinking: targeted retrieval
Prompt
span ��3 ��4 ��5⋯ ⋯ ⋯ ⋯
CoT
trace ⋯ 2. City <marker 2> 3. City <marker 3> 4. City <marker 4> ⋯
Final
answer <Ans> Total: 10
Attention from CoT markers to needle span
Needle
1 2 3 4 5 6 7 8 9 10⋮
Marker 2
92%
Marker 3
89%
Marker 4
90%⋮
Relative mass 0% 50% 100%
C Non-thinking ThinkingNCC Accuracy: 46% NCC Accuracy: 98%
PC1
PC2
PC3 PC1
PC2
PC3
1
2
3
4
6
5
8
9
10
7
1
9 876
5
4
3
2
10Figure 1: Two retrieval mechanisms and contrasting representations. A. Non-thinking
distributes final-query attention across prompt needles. B. Thinking targets successive needles as
its trace progresses. C. PCA projections of needle end representations, colored by running count-
index, with numbered centroids. Held-out nearest-centroid accuracy after whitened 16-component
PCA is 46% for Non-thinking and 98% for Thinking. Attention and representations are based on
Qwen3-8B with 10K-token inputs.2
<think></think> tag before the final-answer count.1
Current mechanistic understanding is limited for long-context inference and CoT reasoning.
First, established analysis in in-context learning and steering mostly works for short contexts, as
models become brittle in long contexts (Liu et al., 2024). Second, in contrast to static single-token
output scenarios, CoT amounts to a dynamic procedure: starting from an input prompt s1:t, a
model emits tokens st+1, st+2, . . . one by one, which iteratively grows the context s1:t → s1:(t+1) →
s1:(t+2) → · · · .
To address the difficulties, we use counting as a simple yet informative case study. Roughly
1In newer models such as Qwen3 and Gemma-4, one checkpoint supports both Non-thinking and Thinking modes
with an on/off switch.
2An interactive 3D visualization is available at https://anonymous.4open.science/r/count-state-geometry-s
upplement-3B2F/index.html. Click “JS off” to enable interaction or download and open it locally.
2
speaking, the representations (or hidden states) at needle positions move along a curve as the
needle-count index progresses, both for prompt needles and CoT needles3. We use counter state for a
distributed representation of counting progress. Running index labels progress at prompt needles or
trace items; final count labels the total at the answer query, whose representation we call the answer
state. For deeper understanding, we ask the following questions. Q1 (internal mechanism): what
attention mechanisms do the two modes use for retrieving needles? Q2 (representation geometry):
how compact are the representations over needle tokens? Q3 (counter-state evolution): do evolving
counter-state representations causally guide subsequent retrieval and final count prediction?
Overall, our key finding is that two distinct mechanisms exist. Non-thinking models depends on
broad retrieval: they broadly attend to all prompt needles at the answer token but produce noisy
representations and unreliable counts. Thinking models depends on targeted retrieval: they
attend to and enumerate needles one by one in CoT traces, thereby improving the count accuracy.
Fig. 1 shows representative illustration for both modes; see A for details. Below, we summarize our
main contributions.
1. A comprehensive comparison across model families. Across needle counts, prompt length,
and model families, needle counts and context lengths hurt model accuracy for Non-thinking
models much more than Thinking models. (Sec. 3)
2. A mechanistic contrast between the two modes. We answer Q1 and Q2 by showing that
Non-thinking models collect noisy representations at lower layers through broad retrieval, while
thinking models develop compact representations through targeted retrieval. For Q3, our causal
intervention results support evolving count states in CoT traces (Sec. 4–5).
3. A controlled experiment on the emergence of two mechanisms. We train small trans-
formers from scratch under autoregressive losses, with or without CoT traces, which controls
either broad retrieval emerges or targeted retrieval emerges. (Sec. 6)
2 Related work
Our mechanistic analysis of long-context counting connects three literatures and offers a unified
account—how needles are retrieved from context, how counts are encoded geometrically, and how
models maintain and update states during CoT reasoning.
Long-context retrieval. NIAH tests isolate fact retrieval from distractor text (Kamradt, 2023),
while RULER, LongBench, and Counting-Stars extend evaluation to multiple facts and aggregation
(Hsieh et al., 2024; Bai et al., 2024; Song et al., 2025). While Wu et al. (2025) identify specialized
retrieval heads, they do not fully explain long-context failures such as Lost-in-the-Middle (Liu et al.,
2024). This limitation motivates our counting study, where we contrast representation compactness
between broad retrieval and targeted retrieval, thus providing a representation-level account of long-
context retrieval.
Counting geometry. Existing mechanistic work identifies low-dimensional curved manifolds
that encode counts or circular calender features (Gurnee et al., 2025; Engels et al., 2025; Kan-
tamneni and Tegmark, 2025; Karkada et al., 2026). Using causal interventions, Hasani et al. (2026)
identify internal counters in text and vision, but its study is mostly limited to simple item-counting
tasks. However, connecting counting geometry to model behavior is challenging, as accurate linear
3We exclude self-reflection in CoT traces, as detailed in Sec. E.1.
3
decoding of counts does not imply correct output (Garcia, 2026). Our work combines layer-wise
geometric analysis with causal interventions to detail the internal pathway for counting.
CoT reasoning and state-tracking mechanism. Despite theoretical benefits of CoT reasoning
(Feng et al., 2023; Merrill and Sabharwal, 2024; Malach, 2024), the mechanism of CoT reasoning
in practice remains largely unsettled, partly due to the difficulty of dynamically growing contexts.
Prior work on Bayesian belief states for in-context learning (Shai et al., 2024; Bigelow et al., 2025;
Yan et al., 2026) is indicative of a general state-tracking mechanism, but current understanding for
CoT reasoning is either limited to toy settings (Zhang et al., 2025; Li et al., 2025; Huang et al.,
2025; Forner et al., 2026; Wang et al., 2026), or based on coarse-grained analysis (Yang et al., 2026).
Our work provides evidence that pretrained LLMs maintain and iteratively update count states
while retrieving sparse records from long distractor passages.
3 Behavioral comparison between the two modes
We evaluate Non-thinking and Thinking on our long-context counting NIAH task (counting city–
score records in distractor text) varying target count N (1–20) and prompt length L (1k–20k tokens)
across 12 open models. Most models have a thinking/nonthinking switch in a single checkpoint;
GLM and Ministral use separate checkpoints. Figure 2 summarizes exact-answer accuracy and
descriptive fits; models, prompts, and scoring are detailed in Appendix C.
Qwen3 Gemma-4 Nemotron GLM† Ministral†
L M 4B 8B 14B 32B E4B 12B 26B-A4B 31B v2-9B 3-4B 4/Z1-9B 3-8B
1k Non-thinking 53.3 73.3 0 33.3 16.7 0 76.7 10 26.7 56.7 0 86.7
Thinking 100 100 100 100 100 100 100 100 93.3 76.7 100 100
20k N 0 23.3 26.7 16.7 0 0 0 10 23.3 26.7 6.7 93.3
Thinking 73.3 83.3 93.3 93.3 33.3 66.7 80 86.7 16.7 23.3 26.7 46.7
Table 1: Parsed exact accuracy (%), N = 10, over 30 paired seeds. †Separate checkpoints.1 2 3 5 10 20
Target count N
0%
25%
50%
75%
100%
Exact accuracy
A Non-thinking
1 2 3 5 10 20
Target count N
B Thinking
0 25 50 75 100
Length L (k tokens)
0%
25%
50%
75%
100%
C Qwen3-32B
0 25 50 75 100
Length L (k tokens)
D Gemma-4-31B
N: 3 5 8 10 15 20
Non-thinking
Thinking
L (tokens): 1k 2k 3k 5k 8k 10k 15k 20k
Figure 2: Counting accuracy across counts and context lengths. A,B. Non-thinking and
Thinking at 1k–20k tokens: observed medians (circles) and fits (lines) across 12 comparison groups;
colors denote length. C,D. Qwen3-32B and Gemma-4-31B: fitted medians across 14 counts using
1k–100k fits; dotted lines mark 20k. Error bars and bands show interquartile ranges across groups
(A,B) or counts (C,D).
4
[TODO: Use default smoothing and draw a new figure.]
Thinking alleviates the difficulty of counting many records.
Longer contexts remain difficult in both modes.
What the fits say about context length. Let EN,L be the error rate of reasoning models in
Panel C and D at needle N and context length L. We want to explain the trend of EN,L with
regard to N and L. We can try to fit
EN,L ∼ α + βN L
And report the fit quality (R2). A theoretical explanations is
[TODO: It’s better if we could have some theoretical insights about the law, maybe
just some heuristic hypothesis.]
4 Non-thinking mode: form, retrieve, and consolidate
Our mechanistic analysis in Sec. 4–5 primarily focuses on Qwen3-8B and Gemma-4-E4B with
approximately 10k-token prompts. Throughout, layer 1 denotes the first Transformer block. We
extended our analysis to additional settings: (i) other retrieval tasks such as localizing kth-retrieval
and counting within a specified category (Appendix H), (ii) CoT reasoning without the <think>
tag by using structured enumeration instructions, such as the indexed and bullet lists (Appendix F).
The additional results are consistent with our main findings.
4.1 Broad attention, noisy representations
First, we examine attention patterns at the final-answer query—the last token of the supplied
assistant prefix Total:—in our NIAH counting task. A subset of heads concentrates attention on
needle spans, consistent with prior work on retrieval heads (Wu et al., 2025). These heads distribute
attention across multiple needles, although individual heads exhibit position preferences (Fig. 3A).1 4 7 10
Needle index (N = 10)
28,19
29,20
24,30
24,14
24,29
25,17
Head (layer, index) Qwen
1 4 7 10
Needle index (N = 10)
30,5
36,3
36,8
36,2
36,4
30,3
Gemma
1 11 21 31
Layer
0.0
0.2
0.4
0.6
Retrieval score Top-32
Qwen
6 18 30 42
Layer
0.0
0.2
0.4
0.6 Top-6
Gemma
0% 10% 20% 25%
Share of needle attention
0% 10% 20% 25%
Share of needle attention
A Attention across needles B Retrieval by layer
Selected heads Other heads
Figure 3: Broad retrieval in Non-thinking models. A. Needle-attention shares for each
model’s six highest-ranked heads, normalized within each N = 10 prompt and averaged over 20
discovery seeds. B. Full-span retrieval scores across counts 2–10; highlighted points mark the frozen
Qwen Top-32 and Gemma Top-6 sets. Gemma includes global-attention layers only.
5
To quantify both the amount and breadth of needle-directed attention, let Ah(q, s) denote head
h’s attention from query q to key s. At the answer query qA, the attention mass on needle span Sj
is mhj = ∑
s∈Sj Ah(qA, s). Across J needles, define the total mass Mh = ∑
j mhj and normalized
shares phj = mhj /Mh for Mh > 0. The broad retrieval score is
Bh = Mh
exp(Hh)
J , Hh = −
J∑
j=1
phj log phj . (1)
Here, exp(Hh) is the effective number of attended needles: it equals k when attention is uniform
over exactly k needles. Dividing by J gives effective coverage, which reaches 100% for uniform
attention across all needles. Thus, Bh rewards both substantial needle-directed attention and
broad coverage. We set 0 log 0 = 0 and Bh = 0 when Mh = 0. Across discovery prompts with 2–10
needles, mean effective coverage is 81.2% for Qwen’s Top-32 heads and 80.3% for Gemma’s Top-6
heads. High-scoring heads concentrate mainly at Qwen L22–29 and Gemma L30–36 (Fig. 3B).
How well do prompt-needle representations encode counts? We next examine whether
needle end states encode each needle’s running index—the number of needles encountered so far.
Ridge regression reads out this index with high confirmation R2 (0.945/0.842 for Qwen/Gemma
at L17/L22). However, predictive accuracy alone does not establish that the decoded direction
controls the model’s count. Motivated by the count-steering results of Hasani et al. (2026), we
test ridge-based linear steering at the last needle span. Across layers, it fails to reliably increase
or decrease the answer in the intended direction (ten initially correct N = 3 prompts per model;
Appendix D.2).
We therefore use PCA to describe representation geometry and nearest-centroid classification
(NCC) to quantify running-index separability, with discovery NCC determining the displayed layers
(Qwen L17/Gemma L22; Appendix D.2). Three components of a separate PCA on class centroids
capture 98.4%/95.3% of their variance, yet confirmation NCC accuracy is only 42%/39%. Thus,
low-dimensional centroid structure and high regression R2 coexist with substantial overlap between
index classes. PCA and NCC characterize this geometry; they do not by themselves establish causal
use.
We also test sensitivity to the opening instructions and needle domain. Decodable count infor-
mation does not guarantee robust transfer across needle types. Removing the opening instructions
retains similar running-index centroid configurations at the selected layers. Replacing city needles
with flower needles lowers frozen answer-state nearest-centroid accuracy from 67% to 50% for Qwen
and from 58% to 43% for Gemma (Appendix D.2).
4.2 The form-retrieve-consolidate mechanism
We next test how needle span information contributes to the final count through causal interventions
at needle sites, retrieval heads, and the answer query. These experiments support a form–retrieve–
consolidate pathway across layers.
6
High layer
Mid layer
Low layer
Tokens
Positions
N1 N2 N3 N10 <Ans>
T
Total: 8
Form
Retrieve Consolidate
A Non-thinking mechanism
1 11 21 31 41
Intervention layer
0%
20%
40%
60%
Effect
Qwen Gemma
Restore
Corrupt
Qwen Gemma
0%
20%
40%
60%
Ablation effect
4%
55%
6%
25%
K = 32 K = 6
Original Random Top-K
1 11 21 31 41
Intervention layer
0%
20%
40%
60%
80%
State-transfer effect Qwen Gemma
B Record-span patching C Head ablation D Answer-state patchingFigure 4: The form–retrieve–consolidate pathway. A. Mechanism schematic. B. Clean-to-
corrupted restoration (solid) and corrupted-to-clean patching (dashed) of complete needle spans.
C. Retrieval-head ablation versus layer-matched random and original-output controls. D. Answer-
state transfer toward the source count.
Form: noisy running count index forms in shallow layers. Shallow layers form contextual
representations at needle spans that reflect each needle’s running index—the number of needles
encountered so far. These representations remain noisy and overlap across indices. To test their
contribution to the answer, we patch activations from a source run into a target run (Heimersheim
and Nanda, 2024). Clean inputs are unmodified, regardless of answer correctness; corruption re-
places needles with length-matched ordinary text. Restoring clean needle span states into corrupted
targets, or reversing this direction, gives large shallow-layer effects (47–50% at L1), falling below 5%
by Qwen L23 and Gemma L18 (Fig. 4B). Needle-site interventions thus affect the answer primarily
before these boundaries.
Retrieve: Broad retrieval collects needles in middle layers. At the answer query, broad
retrieval heads attend to multiple needle spans and combine their information into the represen-
tation at the answer position. To test this role, we ablate the frozen head banks at this query,
producing normalized absolute count changes of 54.5% for Qwen and 24.7% for Gemma, versus
4.0% and 5.7% for layer-matched random banks (Fig. 4C). Top-k sweeps and initially correct-input
controls are in Appendix D.3.
Consolidate: answer states consolidate count information in deep layers. We interpret
the deeper layers as integrating the retrieved needle information into an answer state that guides
the final count prediction. To test this role, we patch answer states between prompts with different
counts. Predictions shift toward the source count, with transfer effects increasing in deep layers
and reaching 59% for Qwen and 73% for Gemma in the single-layer screen (Fig. 4D). Removing
count-aligned components at retrieval and answer sites also reduces restoration more than removing
norm-matched orthogonal components (Appendix D.3).
7
5 Thinking mode: retrieve, update, and read
For Thinking mode, we examine how Qwen and Gemma count through traces that enumerate
prompt records in passage order, studying retrieval and state representations at successive steps.
5.1 Targeted attention, compact representations
During Thinking, the thinking trace creates successive queries for retrieving prompt records. We
examine attention at the token immediately before each trace item. The illustrated Qwen and
Gemma heads preferentially attend to the next record, producing attention patterns that advance
with enumeration (Fig. 5A).1 4 7 10
Needle
0
1
2
3
4
5
6
7
8
9
Marker
Qwen · L25H30
1 4 7 10
Needle
0
1
2
3
4
5
6
7
8
9
Gemma · L30H5
1 11 21 31
Layer
0.0
0.2
0.4
0.6
Targeted score Th Top-128
Qwen
6 18 30 42
Layer
0.0
0.2
0.4
0.6 Top-6
Gemma
0% 50% 100%
Share of needle attention
0% 50% 100%
Share of needle attention
A Attention from CoT markers B Retrieval by layer
Ablated Top-K Other heads
Figure 5: Targeted retrieval in Thinking. A. Needle-normalized attention for one head per
model (N = 10); circles mark needle k + 1 at Marker k. B. Mean Th across discovery seeds;
highlights mark Qwen Top-128 and Gemma Top-6. Gemma includes global-attention layers only.
To quantify this pattern, let qk denote the query preceding trace item k and Sk the complete
span of its corresponding prompt needle. The targeted retrieval score is
Th(qk, Sk) = ∑
s∈Sk
Ah(qk, s). (2)
The score lies between zero and one and measures the fraction of head h’s total attention assigned
to the designated source record. Summing over the complete span includes attention to all tokens
within that record. The heatmaps display needle-normalized shares; Th retains raw attention mass.
We average scores over eligible queries within each discovery seed and then weight seeds equally.
High scores occur in a subset of heads (Fig. 5B). The highlighted Qwen Top-128 and Gemma Top-6
banks are fixed from discovery data for the subsequent causal tests.
How well do CoT-item representations encode counting progress? As in Non-thinking,
we use PCA to display geometry and NCC to quantify running-index separability. Throughout the
paper, geometry display layers maximize discovery NCC accuracy, with logistic accuracy and then
earlier depth breaking ties; preprocessing is fitted within discovery folds. Our exploratory paired
Qwen comparison uses 30 shared N = 10 inputs restricted to correct, complete, consecutively
numbered CoT traces, with a secondary 20/10 discovery/confirmation split. At the NCC-selected
layers (Non-thinking L13; Thinking L31), CoT completed-item states form compact index-specific
groups in the PCA display (Fig. 1C). Confirmation NCC is 98% for CoT-item states and 46% for
paired prompt-record endpoints. These results describe the selected trace family.
8
The broader cohort covers counts 1–10 and retains parsed item occurrences without filtering
on final-answer correctness. Discovery NCC selects Qwen L19 and Gemma L17, yielding confir-
mation balanced accuracy of 58.9% and 71.8%, respectively (Appendix E.2). This cohort differs
in count range and trace composition from the paired comparison, so the two sets of scores are
not a controlled measure of the effect of trace format. Explicit numbering and token position may
contribute to readout. PCA and NCC establish geometric structure and separability; the following
interventions test whether these states influence subsequent retrieval and final count prediction.
5.2 The retrieve–update–read mechanism
We examine a retrieve–update–read mechanism in which successive lookups contribute to counter
states and the completed trace supports answer prediction (Fig. 6A). We test these functions with
head ablations and state interventions.A Thinking mechanism
States
Tokens
Positions
h (ℓ)
τk
Nk
τk
Hk − 1
ek − 1
tk − 1
hqk
query
qk
Hk
item end
tk
hqk + 1
query
qk + 1
HN
eN
tN
aT
⟨Ans⟩
T
Counter state
Terminal
Retrieve
Guide
State update
Repeat
⋯
⋯
Read
Total: N
B Head ablation
Ablation effect
Next item
Final count
0%
50%
100%
10%
60%
7%
80%
Qwen Gemma
0%
50%
100%
37%
100%
57%
100%
K = 128 K = 6
C Counter-state patching
Mumbai → Islamabad → Osaka → Lima → ⋯
Original ... Mumbai Islamabad
Target state after Islamabad
Patched ... Mumbai Osaka → Lima → ⋯
Stepwise success
Model k + 1 k + 2 k + 3 k + 4
Qwen 25/30 25/25 16/16 16/16
Gemma 21/30 20/21 12/12 12/12
D Answer-state patching
1 11 21 31 41
Intervention layer
0%
20%
40%
60%
80%
100%
Target-count adoption
Original Random Top-K Qwen Gemma
Figure 6: The retrieve-update-read pathway. A. Functional schematic. B. Retrieval-head
ablation versus layer-matched random and original-output controls. C. State transfer in Qwen and
prompted Gemma traces without indices; later columns condition on earlier success and another
item remaining. D. Answer-state transfer toward the source count.
Retrieve: targeted heads support successive lookups. Targeted retrieval heads retrieve
information from the next prompt record as each trace item is generated. To test this role, we
ablate the frozen head banks at the retrieval query and throughout subsequent generation. Across
ten confirmation transitions per model, next-item failure increases by 60 and 80 percentage points,
respectively, versus 10 and 6.7 for layer-matched random banks. Final count failure increases by
100 points in both models, versus 36.7 and 56.7 under random masks (Fig. 6B). The selected
heads therefore contribute to both the next lookup and completion of the count. In a head-count
sweep, ablating 64 Qwen heads leaves next-item accuracy at 9/10 and final count accuracy at 0/10,
showing different sensitivities of these two outcomes (Appendix E.3).
9
Update: counter states guide continued enumeration. At the end of each item, the counter
state encodes counting progress and helps guide retrieval of the next needle. We first hold trace
tokens fixed while masking retrieval heads. Masking changes later item-associated states, and restor-
ing clean states reduces the resulting item-end deviation (Appendix E.3). This establishes sensitiv-
ity to retrieval with visible tokens fixed. To test behavior, we transplant a Target’s completed-item
k state into an aligned Receiver prefix ending at k − 1. Qwen uses natural traces without indices;
Gemma uses the separately prompted FOUND: format. Across ten confirmation seeds per model
and k = 4, 6, 8, the next city follows the Target-implied successor k + 1 in 25/30 Qwen and 21/30
Gemma trials, versus 0/30 and 2/30 self controls (Fig. 6C). Among first-step successes, the fol-
lowing item is correct in 25/25 and 20/21 trials without another patch. The transferred states
thus guide continuation beyond the immediately patched step. These counter states jointly carry
progress and record content.
Read: trace information supports the final count. At the final-answer query, the model
uses information in the completed trace to predict the total count. We test this dependence by
separately blanking prompt-record and trace representations while preserving sequence positions.
Prompt-record blanking leaves exact-count accuracy unchanged at 97% for Qwen and 70% for
Gemma; trace blanking reduces it to 1% and 15% (100 prompts per model; Fig. 16A,B). We then
apply answer-state patching between different-count prompts with correct baseline answers. At
the final layer, greedy outputs match the source count in 39/40 Qwen and 36/40 Gemma directed
pairs (Fig. 6D), while self patches preserve the target’s original count. Finally, restoring clean
target states in the post-terminal suffix reverses 47.1% of the loss in the correct-count score margin
caused by terminal-state patching for Qwen and 76.9% for Gemma (Appendix E.3). This supports
a partial causal pathway through which terminal counter states influence final count prediction.
6 Synthetic Experiment: Emergence of Two Retrieval Mechanisms0 2.5k 5k 7.5k 10k
Training steps
0
20
40
60
80
100
Free-running accuracy (%) Non-thinking
Thinking
0 2.5k 5k 7.5k 10k
Training steps
L1
L2
L3
L4
0 2.5k 5k 7.5k 10k
Training steps
L1
L2
L3
L4
0.00
0.03
0.06
Broad score Bh
0.0
0.5
1.0
Targeted needle mass Th
A Answer accuracy B Non-thinking: broad retrieval C Thinking: targeted retrieval
Figure 7: Learning dynamics of two synthetic counting models. A. Thinking model reaches
95% free-running answer accuracy, compared with 21% for Non-thinking model at training plateau.
B. Non-thinking model develop broad retrieval heads in shallow layers. C. Thinking model develop
targeted retrieval heads in deep layers. The dashed line marks the training-objective change at step
1,500; definitions and evaluation details are given in Appendix A.
10
How do models develop the two distinct mechanisms during training? We present a controlled
experiment where we train 4-layer 8-head NanoGPT models from scratch, following the default
hyperparameters as in Karpathy (2022). The training data are a modified Shakespeare corpus:
each input sequence starts with a query, then a 256-character chunk of Shakespeare text, followed
by an optional CoT trace and then the final count. Both models share the architecture, input
distribution, and training budget. Inputs are a character-shuffled 256-character window from Tiny
Shakespeare with target counts from 1 to 10. For readability, we illustrate the sequence format with
an unshuffled text fragment containing four occurrences of the target characters {T,b,n} (boldfaced
below):
<BOS> <CountChar> T b n <Sep> . . . To be, . . . or not to be. . . .
<Think> <Sep> T <Sep> b <Sep> n <Sep> b </Think> <Ans> <4> <EOS>
The trace lists the matching characters in order, without numbering. The Non-thinking model
outputs <Ans> <4> <EOS> directly after the input, without generating a trace. Each sequence
selects three characters as needles to be counted in the text. See Appendix G.1 for details of
dataset construction and training.
Motivated by overfitting in preliminary full-sequence training experiments on the small corpus,
we adopt a two-stage autoregressive schedule. We train on the full sequence for 1,500 steps, then
restrict the loss to task outputs, with the same final count loss weight in both models. The switching
point is fixed for the reported runs.
The learning dynamics reveal a clear distinction between the two models (Fig. 7). The free-
running count accuracy, measured at the token after <Ans>, clearly separates the two models, as
the Thinking model reaches 95%, whereas the Non-thinking model plateaus at 21%. Further, broad
retrieval heads emerge in the first layer of the Non-thinking model, while targeted retrieval heads
emerge in the last layer of the thinking model.
As before, we apply Eqs. (1) and (2) with J = N target occurrences and singleton spans
Sk = {sk}. Broad retrieval is measured at <Ans>; targeted scores are averaged over the N
teacher-forced trace queries within each input. Both scores are then averaged equally across in-
puts (Appendix G.2). The synthetic models also differ in final count readability; counter-state and
answer-state transplants test their roles in trace continuation and final count prediction, respec-
tively (Appendix G).
This synthetic experiment provides additional insights. First, models trained with enumeration
traces develop targeted retrieval, whereas models trained to answer directly develop broad retrieval.
Second, standard autoregressive training on enumeration-type CoT traces already yields strong
counting accuracy, even without specialized post-training. This reinforces a common belief that
high-quality CoT traces are a key ingredient for strong reasoning capability. This result is consistent
with prior work on learning from intermediate traces (Nye et al., 2021; Zelikman et al., 2022;
Muennighoff et al., 2025).
7 Limitations and Future Work
In this work, we answered our motivating questions Q1 and Q2 directly with head-level and
representation-level measurements. For Q3, we validated our conjecture about evolving count
states using causal intervention. A more direct and stronger evidence would be identifying circuits
that implement the update as a needle is retrieved, which is left as future work.
We used counting as a clean testbed for analyzing long-context reasoning in LLMs. To go
beyond this first-step analysis, a further study could analyze sophisticated reasoning tasks that
11
involve search and branching, and the evolution of multiple states in model representations.
Html version
Reproducibility
Acknowledgments
Y.Z. is partially supported by NSF-DMS grant 2412052 and a Coefficient Giving (formerly Open
Philanthropy) grant. In addition, support for this research was provided by the University of
Wisconsin–Madison Office of the Vice Chancellor for Research with funding from the Wisconsin
Alumni Research Foundation. We also thank Haolin Yang for helpful discussions.
References
Yushi Bai, Xin Lv, Jiajie Zhang, Hongchang Lyu, Jiankai Tang, Zhidian Huang, Zhengxiao Du,
Xiao Liu, Aohan Zeng, Lei Hou, Yuxiao Dong, Jie Tang, and Juanzi Li. LongBench: A Bilingual,
Multitask Benchmark for Long Context Understanding. In Proceedings of the 62nd Annual
Meeting of the Association for Computational Linguistics (Volume 1: Long Papers), pages 3119–
3137. Association for Computational Linguistics, 2024. doi: 10.18653/v1/2024.acl-long.172.
URL https://aclanthology.org/2024.acl-long.172/.
Eric Bigelow, Daniel Wurgaft, YingQiao Wang, Noah Goodman, Tomer Ullman, Hidenori Tanaka,
and Ekdeep Singh Lubana. Belief dynamics reveal the dual nature of in-context learning and
activation steering. arXiv preprint arXiv:2511.00617, 2025. URL https://arxiv.org/abs/25
11.00617.
Joshua Engels, Eric J. Michaud, Isaac Liao, Wes Gurnee, and Max Tegmark. Not all language
model features are one-dimensionally linear. In The Thirteenth International Conference on
Learning Representations, 2025. URL https://proceedings.iclr.cc/paper_files/paper/20
25/hash/d3221cdb27e49d9c1cd35ad254feccfe-Abstract-Conference.html.
Guhao Feng, Bohang Zhang, Yuntian Gu, Haotian Ye, Di He, and Liwei Wang. Towards Revealing
the Mystery behind Chain of Thought: A Theoretical Perspective. In Advances in Neural Infor-
mation Processing Systems, volume 36, 2023. URL https://proceedings.neurips.cc/paper_f
iles/paper/2023/hash/dfc310e81992d2e4cedc09ac47eff13e-Abstract-Conference.html.
Niklas Forner, Marcel K¨uhn, Matthias Thamm, and Bernd Rosenow. Learning dynamics of chain-
of-thought state tracking in a solvable transformer model. arXiv preprint arXiv:2606.18164, June
2026. URL https://arxiv.org/abs/2606.18164.
Gabriel Garcia. The right answer, the wrong direction: Why transformers fail at counting and how
to fix it. arXiv preprint arXiv:2605.03258, 2026. URL https://arxiv.org/abs/2605.03258.
Gemma Team. Gemma 4 technical report, 2026. URL https://arxiv.org/abs/2607.02770.
GLM Team, Aohan Zeng, Bin Xu, Bowen Wang, Chenhui Zhang, Da Yin, Dan Zhang, Diego Rojas,
Guanyu Feng, Hanlin Zhao, et al. ChatGLM: A family of large language models from GLM-130B
to GLM-4 all tools, 2024. URL https://arxiv.org/abs/2406.12793.
12
Rhys Gould, Euan Ong, George Ogden, and Arthur Conmy. Successor heads: Recurring, inter-
pretable attention heads in the wild. In The Twelfth International Conference on Learning
Representations, 2024. URL https://openreview.net/forum?id=kvcbV8KQsi.
Wes Gurnee, Emmanuel Ameisen, Isaac Kauvar, Julius Tarng, Adam Pearce, Chris Olah, and
Joshua Batson. When Models Manipulate Manifolds: The Geometry of a Counting Task. Trans-
former Circuits Thread, 2025. URL https://transformer-circuits.pub/2025/linebreak
s/index.html. Original 2025 Transformer Circuits publication; arXiv version posted January
2026.
Hosein Hasani, Amirmohammad Izadi, Fatemeh Askari, Mobin Bagherian, Sadegh Mohammadian,
Mohammad Izadi, and Mahdieh Soleymani Baghshah. Understanding Counting Mechanisms in
Large Language and Vision-Language Models. In Proceedings of the IEEE/CVF Conference on
Computer Vision and Pattern Recognition, pages 5125–5133, 2026. URL https://openaccess
.thecvf.com/content/CVPR2026/html/Hasani_Understanding_Counting_Mechanisms_in_
Large_Language_and_Vision-Language_Models_CVPR_2026_paper.html.
Stefan Heimersheim and Neel Nanda. How to use and interpret activation patching. arXiv preprint
arXiv:2404.15255, 2024. URL https://arxiv.org/abs/2404.15255.
Cheng-Ping Hsieh, Simeng Sun, Samuel Kriman, Shantanu Acharya, Dima Rekesh, Fei Jia, Yang
Zhang, and Boris Ginsburg. RULER: What’s the real context size of your long-context language
models? In First Conference on Language Modeling, 2024. URL https://arxiv.org/abs/2404
.06654.
Yu Huang, Zixin Wen, Aarti Singh, Yuejie Chi, and Yuxin Chen. Transformers provably learn chain-
of-thought reasoning with length generalization. In Advances in Neural Information Processing
Systems, volume 38, 2025. doi: 10.52202/085713-4230. URL https://proceedings.neurips.
cc/paper_files/paper/2025/hash/b86a195e70f27017c514fa0e5f80595f-Abstract-Confe
rence.html.
Greg Kamradt. Needle In A Haystack. GitHub repository, 2023. URL https://github.com/g
kamradt/needle-in-a-haystack. Original benchmark released in 2023; accessed September 8,
2026.
Subhash Kantamneni and Max Tegmark. Language Models Use Trigonometry to Do Addition.
arXiv preprint arXiv:2502.00873, 2025. URL https://arxiv.org/abs/2502.00873.
Dhruva Karkada, Daniel J. Korchinski, Andres Nava, Matthieu Wyart, and Yasaman Bahri. Sym-
metry in language statistics shapes the geometry of model representations. arXiv preprint
arXiv:2602.15029, 2026. URL https://arxiv.org/abs/2602.15029. ICML 2026.
Andrej Karpathy. nanoGPT. https://github.com/karpathy/nanoGPT, 2022. Character-level
Shakespeare example; accessed September 7, 2026.
Andrej Karpathy. minGPT. https://github.com/karpathy/minGPT, n.d. Includes a character-
level language-modeling example; accessed September 8, 2026.
Belinda Z. Li, Zifan Carl Guo, and Jacob Andreas. (How) do language models track state?
In Proceedings of the 42nd International Conference on Machine Learning, volume 267 of
Proceedings of Machine Learning Research, pages 34429–34452. PMLR, 2025. URL https:
//proceedings.mlr.press/v267/li25r.html.
13
Alexander H. Liu, Kartik Khandelwal, Sandeep Subramanian, Victor Jouault, Abhinav Rastogi,
et al. Ministral 3, 2026. URL https://arxiv.org/abs/2601.08584.
Nelson F. Liu, Kevin Lin, John Hewitt, Ashwin Paranjape, Michele Bevilacqua, Fabio Petroni, and
Percy Liang. Lost in the middle: How language models use long contexts. Transactions of the
Association for Computational Linguistics, 12:157–173, 2024. doi: 10.1162/tacl a 00638. URL
https://aclanthology.org/2024.tacl-1.9/.
Eran Malach. Auto-Regressive Next-Token Predictors are Universal Learners. In Proceedings of
the 41st International Conference on Machine Learning, volume 235 of Proceedings of Machine
Learning Research, pages 34417–34431. PMLR, 2024. URL https://proceedings.mlr.press/
v235/malach24a.html.
William Merrill and Ashish Sabharwal. The Expressive Power of Transformers with Chain of
Thought. In The Twelfth International Conference on Learning Representations, 2024. URL
https://openreview.net/forum?id=NjNGlPh8Wh.
Niklas Muennighoff, Zitong Yang, Weijia Shi, Xiang Lisa Li, Li Fei-Fei, Hannaneh Hajishirzi, Luke
Zettlemoyer, Percy Liang, Emmanuel Cand`es, and Tatsunori Hashimoto. s1: Simple test-time
scaling, 2025. URL https://arxiv.org/abs/2501.19393.
NVIDIA. NVIDIA Nemotron 3: Efficient and open intelligence, 2025a. URL https://arxiv.or
g/abs/2512.20856.
NVIDIA. NVIDIA Nemotron Nano 2: An accurate and efficient hybrid mamba-transformer rea-
soning model, 2025b. URL https://arxiv.org/abs/2508.14444.
Maxwell Nye, Anders Johan Andreassen, Guy Gur-Ari, Henryk Michalewski, Jacob Austin, David
Bieber, Danny Dohan, Aitor Lewkowycz, Maarten Bosma, David Luan, Charles Sutton, and
Augustus Odena. Show your work: Scratchpads for intermediate computation with language
models. arXiv preprint arXiv:2112.00114, 2021. URL https://arxiv.org/abs/2112.00114.
quickgrid. nanogpt. https://github.com/quickgrid/nanogpt, n.d. Reports training on Tiny
Shakespeare; accessed September 8, 2026.
Qwen Team. Qwen3 technical report, 2025. URL https://arxiv.org/abs/2505.09388.
Adam S. Shai, Sarah E. Marzen, Lucas Teixeira, Alexander Gietelink Oldenziel, and Paul M.
Riechers. Transformers Represent Belief State Geometry in their Residual Stream. In Advances
in Neural Information Processing Systems, volume 37, 2024. URL https://proceedings.neur
ips.cc/paper_files/paper/2024/hash/8936fa1691764912d9519e1b5673ea66-Abstract-C
onference.html.
Mingyang Song, Mao Zheng, and Xuan Luo. Counting-Stars: A Multi-evidence, Position-aware, and
Scalable Benchmark for Evaluating Long-Context Large Language Models. In Proceedings of the
31st International Conference on Computational Linguistics, pages 3753–3763. Association for
Computational Linguistics, 2025. URL https://aclanthology.org/2025.coling-main.253/.
Ali Taghibakhshi, Sharath Turuvekere Sreenivas, Saurav Muralidharan, Ruisi Cai, Marcin Cho-
chowski, et al. Nemotron elastic: Towards efficient many-in-one reasoning LLMs, 2025. URL
https://arxiv.org/abs/2511.16664.
14
Fuxin Wang, Amr Alazali, and Yiqiao Zhong. How does unfaithful reasoning emerge from autore-
gressive training? a study of synthetic experiments. arXiv preprint arXiv:2602.01017, 2026. URL
https://arxiv.org/abs/2602.01017.
Wenhao Wu, Yizhong Wang, Guangxuan Xiao, Hao Peng, and Yao Fu. Retrieval Head Mechanisti-
cally Explains Long-Context Factuality. In The Thirteenth International Conference on Learning
Representations, 2025. URL https://openreview.net/forum?id=EytBpUGB1Z.
Hao Yan, Haolin Yang, and Yiqiao Zhong. Task vector geometry underlies dual modes of task
inference in transformers. arXiv preprint arXiv:2605.03780, 2026. URL https://arxiv.org/ab
s/2605.03780.
Hao Yang, Qinghua Zhao, Lei Li, Lingyi Meng, and Mengda Yu. How chain-of-thought works?
tracing information flow from decoding, projection, and activation. In Findings of the As-
sociation for Computational Linguistics: ACL 2026, pages 5166–5199. Association for Com-
putational Linguistics, 2026. doi: 10.18653/v1/2026.f indings- acl.255. URL https:
//aclanthology.org/2026.findings-acl.255/.
Eric Zelikman, Yuhuai Wu, Jesse Mu, and Noah D. Goodman. STaR: Bootstrapping reasoning
with reasoning. Advances in Neural Information Processing Systems, 2022. URL https://arxi
v.org/abs/2203.14465.
Yifan Zhang, Wenyu Du, Dongming Jin, Jie Fu, and Zhi Jin. Finite State Automata Inside
Transformers with Chain-of-Thought: A Mechanistic Study on State Tracking. In Proceed-
ings of the 63rd Annual Meeting of the Association for Computational Linguistics (Volume
1: Long Papers), pages 13603–13621. Association for Computational Linguistics, 2025. doi:
10.18653/v1/2025.acl-long.668. URL https://aclanthology.org/2025.acl-long.668/.
15
Appendix Contents
A Details of the main-text figures 17
B Additional related work 19
C Further details for the behavioral comparison 19
C.1 Prompts and experimental design . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 19
C.2 Evaluation grid and model-level results . . . . . . . . . . . . . . . . . . . . . . . . . . 20
C.3 Long-context observations and non-monotonicity . . . . . . . . . . . . . . . . . . . . 22
C.4 Regression specification and validation . . . . . . . . . . . . . . . . . . . . . . . . . . 22
C.5 Long-context fits and extrapolation . . . . . . . . . . . . . . . . . . . . . . . . . . . . 22
D Further details for the Non-thinking mode experiment 23
D.1 Experimental design . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 23
D.2 Broad retrieval and count representations . . . . . . . . . . . . . . . . . . . . . . . . 23
D.3 Causal tests of the form–retrieve–consolidate pathway . . . . . . . . . . . . . . . . . 27
E Further details for the Thinking mode experiment 29
E.1 Experimental design . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 29
E.2 Targeted attention and compact count representations . . . . . . . . . . . . . . . . . 30
E.3 Causal tests of the retrieve–update–read pathway . . . . . . . . . . . . . . . . . . . . 30
F Further details for the structured enumeration experiment 31
F.1 Experimental design . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 31
F.2 Enumeration trace parsing . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 32
F.3 Count representations . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 32
F.4 Retrieval, continuation, and answer readout . . . . . . . . . . . . . . . . . . . . . . . 32
F.5 Scope controls and limitations . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 32
G Further details for the synthetic experiment 32
G.1 Experimental design . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 32
G.2 Broad and targeted retrieval heads . . . . . . . . . . . . . . . . . . . . . . . . . . . . 36
G.3 Count representations and causal interventions . . . . . . . . . . . . . . . . . . . . . 38
G.4 Learning dynamics of retrieval and counting . . . . . . . . . . . . . . . . . . . . . . . 42
G.5 Relation to the main experiments . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 44
H Further details for additional tasks 44
H.1 Experimental design . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . . 44
H.2 Behavioral comparison between the two modes . . . . . . . . . . . . . . . . . . . . . 46
H.3 Retrieval-head distributions and causal tests . . . . . . . . . . . . . . . . . . . . . . . 47
H.4 Implications for the retrieval mechanisms . . . . . . . . . . . . . . . . . . . . . . . . 50
16
A Details of the main-text figures
This appendix provides panel-level details for the main-text figures, in order of appearance.
Figure 1: retrieval and representations Panels A–B use the same ten-record, approximately
10k-token Qwen3-8B input (seed 1255), selected for a complete CoT trace and distributed Non-
thinking attention. Arrows and marker labels are schematic.
Panel A: prompt attention. Head L29H20 is measured at the final token of the supplied Total:
prefix. The strip sums raw attention in 170 approximately equal-width bins, ab = ∑
t∈Bb αq,t.
Intensity is √min(ab/τ, 1), with τ the 98.5th percentile (≈ 0.099); the colorbar, labeled Attention
mass, reports raw bin mass.
Panel B: successive retrieval. For head L25H30, query qk precedes item k (Marker k − 1); Marker
0 denotes initialization. The three rows show Markers 2, 3, and 4 (k = 3, 4, 5), matching the
schematic. Each cell reports needle-normalized attention,
sk,j =
∑
t∈span(Nj ) αqk ,t
∑10
r=1
∑
t∈span(Nr ) αqk ,t
, k ∈ {3, 4, 5}, j = 1, . . . , 10.
Each row sums to one over the ten complete needle spans; attention to other tokens is excluded
from the denominator. Outlined cells mark the next needle, j = k, with rounded shares of 92%,
89%, and 90% beneath the respective cells. Needle indices indicate occurrence order rather than
token distance, and ellipses indicate omitted queries. The bottom colorbar, labeled Relative mass,
is linear from 0% to 100% and reports each needle’s share of total needle attention; Panel A retains
its different raw-bin-mass mapping. Blue arrows denote attention; dark-orange boxes label query
positions.
Panel C: running-index representations. To reduce variation in trace format and align item-end
representations consistently, we restrict this comparison to traces with a shared numbered format.
Thirty paired N = 10 inputs are restricted to correct, complete, consecutively numbered CoT
traces. Format selection and the secondary 20/10 discovery/confirmation split followed exploration;
this is not a fresh confirmation cohort. Prompt-record endpoints (Non-thinking, L13) and trace-
item endpoints (CoT, L31) yield 46% and 98% nearest-centroid accuracy with 16 whitened PCs.
The display projects 100 confirmation states per mode onto separate discovery-fitted three-PC
bases, with numbered centroids. Discovery NCC layer selection and preprocessing are detailed in
Appendix E.2. Cross-mode distances are not comparable; numbering and position may contribute
to readability.
Figure 2: observed counting accuracy
Figure 3: broad retrieval The discovery cohort has no correctness filter (Table 2); head selec-
tion is detailed in Appendix D.2.
Panel A: needle-attention shares. Cells average the within-prompt shares phj defined above Eq. 1, on
a shared linear 0–25% scale. Needles follow occurrence order; 10% denotes equal shares. Averaged
profiles do not imply uniform attention on individual inputs.
Panel B: layerwise scores. Each point is a head’s mean full-span Bh; both models share the scale.
Highlights retain the frozen head banks. Effective-coverage summaries use the complete banks
across counts 2–10.
17
Figure 4: the causal pathway Protocols and populations are in Appendices D.1 and D.3.
Bands and bars show pointwise 95% seed-bootstrap intervals. Panels B–D measure different effects.
Panel A: mechanism schematic. The diagram summarizes state formation, retrieval, and consoli-
dation; arrows and depths are illustrative.
Panel B: needle span patching. Clean-to-corrupted restoration (solid) and corrupted-to-clean patch-
ing (dashed) measure normalized error reduction and increase, respectively (Eq. 4). Bootstrap
draws pair seeds across directions. Gemma’s mixed-backend restoration limits directional compar-
isons.
Panel C: retrieval-head ablation. Filled circles show selected-bank ablations, diamonds layer-
matched random banks, and hollow circles unmodified runs. Effects are normalized absolute count
changes, | ˆNabl − ˆNclean|/N (Appendix D.3).
Panel D: answer-state transfer. Signed transfer subtracts the paired mean of same-count-source
and self-patch controls (Eq. 5). This is a screening sweep; layerwise effects have not all been
independently confirmed.
Figure 5: targeted attention Panel A: examples and normalization. Both examples use in-
dexed ten-item traces in approximately 10k-token passages (Qwen: seed 1255, L25H30; Gemma:
seed 1240, L30H5). Marker 0 denotes initialization; Marker k follows completed item k. Attention
is normalized over complete needle spans so that each row sums to one, with a shared linear 0–100%
scale. Circles mark the designated next needle.
Panel B: scores and membership. Raw Th is averaged within discovery seed, then across seeds: Qwen
uses post marker queries in adjacent rank before city (15 seeds); Gemma uses p0 item end in
same unit rank before city (19 seeds). The shared scale covers 1,152 Qwen and 56 Gemma
heads. Highlights preserve frozen banks; Gemma’s plotted scores need not reproduce its bank’s
selection ranking.
Figure 6: retrieval and counter states Populations and protocols are in Appendices E.1
and E.3. Target supplies the state transplanted into Receiver.
Panel A: notation and scope. Nk is record k at τk; ek is its trace item; Hk is its counter state at
the completed-item anchor tk, possibly spanning multiple tokens. hqk and aT are retrieval- and
answer-query states. Update summarizes fixed-token retrieval-mask and state-restoration effects;
Read summarizes terminal-state mediation of the final answer. Arrows indicate functional relations,
with the intervention layers and cohorts specified in Appendix E.3.
Panel B: ablation. Ten seeds/model compare persistent masking of the frozen bank (filled circles),
three layer-matched random banks (diamonds, averaged), and unmodified runs (hollow circles).
Effects are percentage-point failure increases; bootstrap draws pair conditions by seed.
Panel C: counter-state transfer. The illustration uses Qwen seed 1307. The table pools forward
k = 4, 6, 8 patches from ten seeds/model; later fractions require preceding success and another item
remaining (Appendix E.3).
Panel D: answer transfer. Every decoder layer reuses 40 directed pairs/model with correct baseline
answers. This sweep extends the existing cohort.
Figure 7: synthetic learning dynamics Each mode uses one four-layer, eight-head Trans-
former trained with seed 1234 (Appendix G).
Panel A: counting accuracy. Eleven pre-specified checkpoints use 100 held-out inputs, ten per count
N = 1, . . . , 10. This single-training-seed comparison has no error bars.
18
Panels B–C: retrieval scores. The same inputs are evaluated every 100 steps, including step 0
(101 checkpoints). Non-thinking uses Bh; Thinking uses teacher-forced query-to-source attention
(Appendix G.2). All 32 heads are ordered by layer, then head; each mode has a fixed raw-score
color scale.
B Additional related work
[TODO: Credit some sources of inspiration of main claims and figures,]
C Further details for the behavioral comparison
C.1 Prompts and experimental design
The behavioral and mechanism experiments share the following city–score counting template. The
placeholder {passage} denotes the complete experimental passage, and {response_instruction}
is replaced by the instruction for the selected mode. Box titles and role labels are annotations;
angle-bracketed output placeholders are literal parts of the instructions sent to the model.
Prompt | Common counting template
User message
You will need to count all city-score audit records in the passage below.
A city-score audit record names one city and gives that city’s numeric score.
<passage>
{passage}
</passage>
How many city-score audit records are in the passage?
{response_instruction}
Prompt | Response instructions
Non-thinking
Do not explain, reason aloud, quote, or list any records.
Your entire response must be exactly one line:
Total: <integer>
Thinking
Reason concisely without repeating or restarting.
Stop as soon as you determine the count, then output exactly one line:
Total: <integer>
The behavioral comparison uses these Non-thinking and Thinking instructions. Structured
enumeration replaces only {response_instruction} with the block in Appendix F.1; its behavioral
and mechanism experiments use identical wording. Appendices D.1 and E.1 list the remaining
protocol-specific changes. All messages use the registered checkpoint’s chat template with add
19
generation prompt=True. The behavioral protocol supplies no additional assistant prefix.
C.2 Evaluation grid and model-level results
Models and comparison groups. We evaluate 12 comparison groups spanning Qwen3-4B,
Qwen3-8B, Qwen3-14B, and Qwen3-32B (Qwen Team, 2025); Gemma-4-E4B, Gemma-4-12B, Gemma-
4-26B-A4B, and Gemma-4-31B (Gemma Team, 2026); NVIDIA-Nemotron-Nano-9B-v2 (NVIDIA,
2025b); NVIDIA-Nemotron-3-Nano-4B (NVIDIA, 2025a; Taghibakhshi et al., 2025); the GLM-4-
9B-0414/GLM-Z1-9B-0414 pair (GLM Team et al., 2024); and the Ministral 3 Instruct/Reasoning
pair (Liu et al., 2026). Qwen3, Gemma-4, and Nemotron-3-Nano-4B use enable thinking to switch
modes; enumeration disables the built-in thinking mode. Nemotron-Nano-v2-9B instead receives
the system message /no think or /think. GLM and Ministral use their paired Non-thinking and
reasoning checkpoints, with the registered system instruction added for Ministral 3 Reasoning.
20
0%
25%
50%
75%
100%
A Qwen3-4B B Qwen3-8B C Qwen3-14B
0%
25%
50%
75%
100%
D Qwen3-32B E Gemma-4-E4B F Gemma-4-12B
0%
25%
50%
75%
100%
G Gemma-4-26B-A4B H Gemma-4-31B I Nemotron Nano 9B-v2
1 2 3 5 10 20
Target count N
0%
25%
50%
75%
100%
J Nemotron-3-Nano-4B
1 2 3 5 10 20
Target count N
K GLM-4/Z1-9B†
1 2 3 5 10 20
Target count N
L Ministral-3-8B pair†
Exact accuracy
L (tokens): 1k 2k 3k 5k 8k 10k 15k 20k
Non-thinking ThinkingFigure 8: Counting accuracy for all 12 comparison groups. Each panel shows exact accuracy
against target count N on a logarithmic horizontal axis; colors denote the eight passage lengths
from 1k to 20k tokens. Circles and solid lines denote Non-thinking; triangles and dashed lines
denote Thinking. Each point averages 30 requests, counting unparseable responses as errors. Lines
are full-grid fits from Eq. (3), with separate coefficients for each group and mode. All 14 counts
and eight lengths are retained, with common axes across panels. † marks GLM and Ministral
comparisons between separate checkpoints; the other panels compare modes within one checkpoint.
logit pNT(N, L) = a + b ln N + cLk,
logit pT(N, L) = ˜a + ˜bN + ˜c ln Lk. (3)
21
C.3 Long-context observations and non-monotonicity
C.4 Regression specification and validation
C.5 Long-context fits and extrapolation
22
D Further details for the Non-thinking mode experiment
D.1 Experimental design
Experiments use Qwen3-8B and Gemma-4-E4B on approximately 10k-token passages. We modify
the common Non-thinking prompt in Appendix C.1 by inserting “Write the count using ordinary
decimal digits, with no space after the colon.” before “Your entire response must be exactly one
line:”, and replacing Total: <integer> with Total:<integer>. After chat-template rendering
with thinking disabled, we supply the assistant prefix Total:; its final token is the answer query.
A needle span is a complete city–score record; its endpoint is its final token. Needle end and
answer-query states are labeled by running index i and final count N , respectively. Layer/head
indices are one-based: Qwen L1–36 and Gemma L1–42.
Table 2 lists the cohorts; default discovery/confirmation seeds are 1234–1253/1254–1263. In-
terventions and controls use matched prompts, with sites and directions fixed before confirmation
where a split is used. Clean means unmodified, regardless of correctness. We writê N for the
generated count, Ns, Nt for source/target counts, and E for the expected count conditional on can-
didate answers 1–10. Effects average counts/pairs within seed, then seeds equally. Unless specified
otherwise, intervals use 10,000 seed-bootstrap draws and are pointwise 95% intervals. Blue/orange
denote Qwen/Gemma; PCA colors denote index/count.
Table 2: Data and splits for Non-thinking experiments, per model unless specified. Eligibility and
invalid-output rules accompany each analysis.
Analysis Data and split
Head scores 20 discovery seeds, N = 2–10: 180 prompts.
Needle end geometry N = 10: 200 discovery endpoints and 100 confirmation endpoints.
Count classification 20 discovery seeds, shared five-fold seed splits. Running index: 200 endpoints
at N = 10; final count: 200 answer-query states at N = 1–10.
Prompt-span steering Ten initially correct N = 3 prompts; all layers.
Cue/domain controls Cue: ten paired seeds 1234–1243 at N = 10. Domain: fit on 20 city-discovery
seeds; test on ten confirmation seeds, N = 1–10, in each domain.
Head ablation 20 seeds 1316–1335, N = 1–5: 100 prompts.
Span patching / serial
tests
Ten confirmation seeds, N = 1–10: 100 prompts. Answer-subspace removal
uses N = 2–10: 90 prompts.
Answer-state patching Screen: seeds 1254–1258, 18 directed pairs per seed. Confirmation: seeds 1259–
1263; correct-input eligibility is supplemented as described below.
D.2 Broad retrieval and count representations
Head selection and complete scores. Mean discovery full-span Bh (Eq. 1) ranks the frozen
Qwen Top-32/Gemma Top-6 banks. Figure 9 includes every measured head; Gemma is restricted
to global-attention layers. Representative attention profiles are in Fig. 3.
23
1 5 9 13 17 21 25 29 32
Head index
1
4
7
10
13
16
19
22
25
28
31
34
36
Layer
1
2
34 5
6
7
8
9
10
11
12
131415 16
17
18
19
20
21
22
23
24
25
26
27
28
29
30
31
32
A. Qwen: all heads
0.0
0.2
0.4
0.6
Broad retrieval score Bh
1 2 3 4 5 6 7 8
Head index
6
12
18
24
30
36
42
Global layer
1
2 34 5
6
B. Gemma: global-attention heads
0.0
0.2
0.4
0.6
Broad retrieval score BhFigure 9: Complete broad-retrieval scores. A. All 1,152 Qwen heads. B. All 56 Gemma
global-attention heads. Cells show mean Bh on 180 discovery prompts, with a shared 0–0.6 scale.
Outlines and numbers mark membership and rank in the Qwen Top-32/Gemma Top-6 banks.
Running-index geometry and final count readout. We compare nearest-centroid classifica-
tion (NCC) and L2 logistic regression (C = 1) across layers using shared five-fold seed splits. Each
fold fits unwhitened PCA32 followed by coordinate standardization for needle end states, and stan-
dardization followed by PCA32 for answer-query states. NCC shrinkage is zero/0.1, respectively.
Layers maximize discovery NCC accuracy, with ties broken by logistic accuracy and then earlier
depth.
24
For running index, this selects Qwen L17/Gemma L22 (discovery NCC 48%/38%). Refitting
on discovery yields confirmation NCC of 42%/39% and ridge R2 = 0.945/0.842 with penalty one in
the same coordinates. A separate PCA of the ten discovery class centroids captures 98.4%/95.3%
of centroid variance in three components: ordered class means coexist with overlapping individual
states. Index also covaries with position. These revised layer choices reuse the existing confirmation
set. Figure 10 compares the two readouts; final count NCC peaks at 67% for Qwen L25 and 59%
for Gemma L30 on discovery folds.1 10 20 30 42
Layer
0%
20%
40%
60%
80%
Classification accuracy
L17
L22
A. Running index
1 10 20 30 42
Layer
0%
20%
40%
60%
80% L25
L30
B. Final count
Qwen Gemma Nearest centroid Logistic
Figure 10: Count readout across layers. A. Running index at needle endpoints. B. Final count
at the answer query. Each uses 200 states and the same 20 discovery seeds and five folds. Solid/-
dashed curves denote nearest-centroid/logistic classifiers; dotted lines mark 10% chance. Labeled
markers identify the NCC-selected layers, with logistic accuracy and then earlier layers breaking
ties.
Linear steering at the last needle. Neither model answers the ten original N = 10 confirma-
tion prompts correctly, so the all-layer scan uses ten initially correct N = 3 prompts/model; Qwen
adds seeds 1264–1265. Every last-needle token receives βσv, where v is the discovery PCA32–ridge
direction mapped to residual space and normalized, β = ±1, and σ is its discovery span-projection
standard deviation. Controls use norm-matched orthogonal-random directions and zero strength.
Gemma’s answers remain unchanged. Under +1, Qwen changes its answer seven times at L19–20:
six from 3 to 2 and one from 3 to 4. Random controls also induce underestimation; zero controls
preserve outputs. The intervention provides no reliable directional control.
Opening-cue and needle-domain controls. Removing the two opening task-definition sen-
tences preserves the passage, final question, and answer format. At the running-index layers se-
lected above, PCA fitted jointly to both conditions shows similar centroid configurations (Fig. 11A–
B; linear CKA between running-index centroids in the original hidden space is 0.999/0.975). This
comparison concerns geometry under cue removal.
For domain transfer, city becomes flower or animal throughout the prompt and records. City-
only discovery NCC selects Qwen L24/Gemma L39 using standardization and whitened PCA16
without NCC shrinkage, with the same tie rule; this differs from the PCA32 layer scan. Frozen
classifiers are evaluated on confirmation prompts in each domain (Table 3). Flower transfer lowers
answer-query accuracy in both models. For visualization, a separate city-discovery standardization
25
and unwhitened PCA3 are applied unchanged to city, flower, and animal states (Fig. 11C–D).A. Qwen L17 PC1-3: 57.3%
PC1
PC2
PC3
B. Gemma L22 PC1-3: 44.2%
PC1
PC2
PC3
C. Qwen L24 PC1-3: 59.4%
PC1
PC2
PC3
D. Gemma L39 PC1-3: 68.7%
PC1
PC2
PC3
1 10
Opening cue: needle end states
Needle domain: answer-query states
Running index / final count
Cue present Cue absent
City Flower Animal
Figure 11: Cue and domain controls. A,B: 100 needle end states per condition in the first three
components of a jointly fitted unwhitened PCA6. C,D: 100 answer-query states per domain (city,
flower, animal) in a city-discovery-fitted PCA3. Small points are states; connected large markers are
class means. Circles/triangles denote cue present/absent in A,B; circles/triangles/squares denote
city/flower/animal in C,D. Percentages give fitting-population variance explained. Conditions share
the projection and display scale within each panel.
Table 3: Frozen city-trained count readout. Nearest-centroid accuracy on 100 confirmation
prompts per topic (N = 1–10; ten seeds). Chance is 10%.
Model City Flower Animal
Qwen L24 67% 50% 56%
Gemma L39 58% 43% 53%
26
D.3 Causal tests of the form–retrieve–consolidate pathway
Form: needle span patching. Corruption replaces needles with equal-token-length ordinary
text. At each layer, restoration copies clean post-block span states into the corrupted target;
reverse patching copies corrupted states into the clean target. Normalized error reduction/increase
is
erestore = |Ecorrupt − N | − |Erestored − N |
N , ecorrupt = |Epatched − N | − |Eclean − N |
N . (4)
Figure 4B reports both restoration and corruption effects, which weaken at deeper layers. Endpoint-
only and token-budget/structure-matched ordinary-region restoration stay within 1.5 percentage
points of zero relative to their corresponding corrupted baselines.
Retrieve: head ablation. We zero head contributions at the answer query and generate greedily,
measuring |̂ Nablated −̂ Nclean|/N . The K ∈ {1, 2, 4, 8, 16, 32} sweep and Gemma’s additional K = 6
run use the same 100 prompts per model. At each dose, three random banks match per-layer
head counts, sample without replacement within banks, and may overlap ranked heads. Replicates
average within prompt. One Gemma random output of 11 is excluded under the specified valid
range 0–10; its other two replicates remain. Figure 12 shows the dose sweeps, including the finalized
Qwen Top-32/Gemma Top-6 banks. On 87 Qwen/63 Gemma initially correct prompts, equal-seed
correct-to-wrong rates are 67.5%/8.8% for ranked/random Qwen K = 32, and 33.3%/12.5% for
Gemma K = 6.1 2 4 8 16 32
Number of ablated heads
0%
20%
40%
60%
Effect
A. Qwen: head ablation
Ranked Random
1 2 4 6 8 16 32
Number of ablated heads
0%
20%
40%
60%
Effect
B. Gemma: head ablation
Ranked Random
Figure 12: Retrieval-head ablation. A: Qwen; B: Gemma. Ranked heads (solid circles) versus
layer-matched random banks (dashed diamonds). Effect is the absolute change in generated count
divided by the true count N . Bands show seed-bootstrap intervals.
Consolidate: answer-state patching and removal. Single-layer and cumulative-from-layer
patches screen counts 0–10 with offsets ±1, ±3, ±5, measuring signed transfer
T =̂ Npatched −̂ Nbaseline
Ns − Nt
. (5)
Invalid outputs contribute zero. Same-count/self controls retain the matched pair’s nonzero denom-
inator; self controls may reuse preflight-validated baselines. Transfer increases in deep layers with
small control effects (Fig. 13); the main figure subtracts their paired mean.
27
1 11 21 31
Intervention layer
0%
40%
80%
Signed count transfer A. Qwen: answer-state controls
Different count
Self patch
Same count
1 11 21 31 41
Intervention layer
0%
40%
80%
Signed count transfer B. Gemma: answer-state controls
Different count
Self patch
Same countFigure 13: Answer-state patching controls. A: Qwen; B: Gemma. Different-count (solid),
same-count (dashed), and self (dotted) single-layer patches, with seed-bootstrap intervals.
Confirmation requires positive transfer in both directions, adjusted effect ≥ 0.15, at least four
positive seeds/two positive anchor pairs, and ≥ 95% valid outputs. Correct-input pairs use five
supplemented seed clusters per displacement/direction. Source-count matches total 1628/1686 for
Qwen and 1809/1884 for Gemma across selected single-layer/cumulative patches (Fig. 14A). Invalid
outputs fail; seed-bootstrap intervals recompute these pooled ratios.
For removal, fit rank-three U to centered discovery answer-state centroids (N = 1–10) and apply
h′ = h − U U ⊤(h − μ), with discovery mean μ. Orthogonal within-count-residual controls match
removal norm within 5%. Panel B shows additional normalized error, (|̂ Naligned −N |−|̂ Northogonal −
N |)/N ; unparseable outputs receive error ten before normalization. Late-layer effects survive Holm
correction across layers within each model/population, including initially correct inputs.−5 −3 −1 +1 +3 +5
Source count − target count
80%
90%
100%
Source-count match A. Correct-input transfer
1 11 21 31 41
Intervention layer
0%
10%
20%
30%
Effect
B. Answer-subspace removal
Qwen Gemma
Figure 14: Answer-state transfer and removal. A: source-count match. B: normalized excess
error from aligned removal. Seed-bootstrap intervals (50,000 draws in B).
Connecting the three stages. Serial tests restore needle states, then remove discovery-fitted
rank-three retrieval/answer components against norm-matched orthogonal controls. The original
needle/retrieval/answer layers remain 9 → 24 → 30 for Qwen and 10 → 30 → 38 for Gemma,
independently of the revised NCC display layers. Banks are Qwen L24 H11,13,14,29,30,31,32 and
Gemma L30 H3/H5; the latter follows the Top-6 extension and is frozen before follow-up outcomes.
Let e(X) = |EX − N |/N ; S/O restore needle/ordinary states in the same corrupted target, and
a/o denote aligned/orthogonal retrieval (R) or answer (A) removal. Figure 15A reports restoration
28
e(O) − e(S) and removal effects e(SRa) − e(SRo), e(SAa) − e(SAo). Retrieval removal increases
normalized error by 12.6/9.8 percentage points for Qwen/Gemma; answer removal increases it by
53.9/52.0, supporting both components’ causal contribution.
Panel B gives interaction [e(SRaAa)−e(SRoAa)]−[e(SRaAo)−e(SRoAo)] and remaining repair
e(O) − e(SRaAa). Negative interaction means that retrieval removal has a smaller additional effect
when the answer component is also removed. Remaining repair is slightly negative: joint removal
leaves more error than ordinary-region restoration. These effects share the true-count denominator
N ; they are not fractions of the restoration effect.Span repair Retrieval
removal
Answer
removal
−20%
0%
20%
40%
60%
Effect
A. Sequential interventions
Interaction Remaining repair
−20%
0%
20%
40%
60%
Effect
B. Joint intervention
Qwen Gemma
Figure 15: Serial interventions across the three stages. A: restoration and retrieval/answer
removal effects. B: interaction and remaining repair. All contrasts use absolute expected-count
error divided by N before averaging; both panels share the same percentage scale. Bars show
seed-bootstrap intervals.
E Further details for the Thinking mode experiment
E.1 Experimental design
In this section, Qwen3-8B and Gemma-4-E4B use approximately 10k-token passages, the Thinking
template (Appendix C.1), thinking enabled, and no assistant prefill. Needles are prompt records;
trace items are generated mentions. Query qk precedes item k (Marker k − 1 in Fig. 5); Hk
is anchored at item completion and may span multiple tokens. The answer query precedes the
numeral. Layers/heads are one-based (Qwen 36/Gemma 42 layers).
Gemma control without indices. This auxiliary condition uses the replacement instruction
below and supplies FOUND: followed by one space as the assistant prefix. The passage, count
question, and enabled thinking mode remain the same. This is an explicitly prompted format
control, so its traces are not treated as spontaneous behavior under the principal native prompt.
29
Prompt | Gemma control: replacement response instruction
During reasoning, write each matching record on one line using exactly:
FOUND: <city> | score <score>
Always use the same literal marker FOUND:. Do not number records, use ordinal
words, item/record/excerpt indices, mention how many have been found, or write a
running subtotal. Do not write a preamble, recap, verification, or explanation.
Immediately after the final FOUND: line, output exactly one line:
Total: <integer>
Your assistant response has already begun with the literal text ’FOUND: ’;
continue that first line directly with the first city and score.
Parsing and eligibility.
E.2 Targeted attention and compact count representations
E.3 Causal tests of the retrieve–update–read pathway
Retrieval-head ablation and head-count dependence.
Retrieval-sensitive trace states.
Counter-state transfer.
Trace information and answer-state patching.
30
Original Prompt
blank
Trace
blank
0%
50%
100%
Exact-count accuracy
A. Qwen: answer sources
Original Prompt
blank
Trace
blank
0%
50%
100%
Exact-count accuracy
B. Gemma: answer sources
0 2 4 6
Count-score margin change
Natural
damage
Suffix
residual
Suffix
mediated
Query
mediated
C. Qwen: terminal pathway
0 2 4 6
Count-score margin change
Natural
damage
Suffix
residual
Suffix
mediated
Query
mediated
D. Gemma: terminal pathwayFigure 16: Trace dependence and terminal mediation. A,B: exact-count accuracy after
Original, prompt-record-blanked, or trace-blanked generation (100 prompts/model). C,D: natural
terminal damage, residual damage after suffix reset, and suffix-/query-mediated damage (86 com-
mon pairs/model), in count-score margin units. Query and suffix effects are nested alternatives.
Intervals use 10,000 seed-bootstrap draws, random seed 20260912. Blue denotes Qwen and orange
Gemma.
Terminal-state mediation.
Additional controls and implementation checks.
F Further details for the structured enumeration experiment
F.1 Experimental design
Structured enumeration uses the common template in Appendix C.1 and the replacement response
instruction below. The indexed and bullet conditions differ only in {item_format}. These instruc-
tions are identical in the behavioral and enumeration mechanism experiments; native thinking is
disabled and no assistant prefix is supplied.
31
Prompt | Structured enumeration: response instruction
Shared instruction
List each occurrence once, in passage order.
{item_format}
Use only actual values from the passage; do not output placeholders or angle
brackets.
Then report the number listed:
Total: <integer>
Do not include any other text.
Indexed item format
Begin the first item with "1. ", the second with "2. ", and continue with ordinary
digits.
After each number, write the actual city name, then ": ", then the actual numeric
score.
Bullet item format
Begin each item with "-", then write the actual city name, then ": ", then the
actual numeric score.
F.2 Enumeration trace parsing
[TODO: Use this to claim that the model only have some types of reasoning is “smart”.]
F.3 Count representations
F.4 Retrieval, continuation, and answer readout
F.5 Scope controls and limitations
G Further details for the synthetic experiment
Our experiment adapts the small-decoder training setup of nanoGPT, whose character-level ex-
ample trains on Tiny Shakespeare (Karpathy, 2022). Related public implementations include
minGPT’s character-level language model (Karpathy, n.d.) and a nanoGPT reproduction on the
same corpus (quickgrid, n.d.). We extend this setup with target-character queries and enumeration-
trace supervision to study how retrieval and counting functions develop in a controlled setting.
G.1 Experimental design
Task and data construction. An input consists of a target set S containing three distinct
characters and a sequence x = (x1, . . . , x256). Let p1 < · · · < pN be the positions for which xpk ∈ S,
and write ak = xpk . The required answer is the total number of occurrences, N = ∑256
j=1 1{xj ∈ S},
with N ∈ {1, . . . , 10}. Matching is case-sensitive, and repeated appearances of the same character
are counted separately.
We split Tiny Shakespeare into contiguous training, validation, and test regions with an 80/10/10
allocation after reserving two 255-character guard intervals. Every source window lies within one
32
region. A fixed pool contains 100 target sets, selected using training-region character frequencies;
each set has combined frequency at most 10/256, with sampling stratified across 20 frequency
bins. During training, a maximum-entropy distribution over feasible (target set, count) pairs gives
uniform set and count marginals. Conditional on a pair, a valid source-window start is sampled
uniformly. We then randomly permute the 256 characters and shuffle the order of characters in the
query. The permutation preserves the count and defines the source order used by the trace.
Sequence format. Corpus characters and structural tags are individual tokens; each final count
also has its own atomic token. Both modes receive the same query and input format. Non-thinking
directly predicts the answer, whereas thinking enumerates the matching characters in source order
without explicit indices:
prompt: <BOS> <CountChar> S1 S2 S3 <Sep> x,
Non-thinking: <Ans> <N > <EOS>,
thinking: <Think> <Sep> a1 · · · <Sep> aN
</Think> <Ans> <N > <EOS>.
Here S1, S2, S3 denote the displayed query order. As in the main text, blue marks the query prefix,
vermilion the trace, and green the answer; target occurrences are bold. Table 4 illustrates absent
query characters, repeated occurrences, and adjacent occurrences (A–C).
33
Table 4: Examples of synthetic inputs. Three actual test-region inputs and their expected
outputs in both modes. The input characters are randomly permuted, so these excerpts do not
preserve words or sentences. Within each example, both modes receive the same query prefix and
256-character input. Excerpts retain every target occurrence and nearby non-target characters; el-
lipses omit only non-target characters. Positions are one-based. Boldface marks target occurrences,
denotes an input space, and \n denotes an input newline.
A. One occurrence (N = 1)
Query <BOS> <CountChar> S c D <Sep>
Shuffled input excerpt . . . ,rc G . . .
Target positions 232
Counts by character S: 0, c: 1, D: 0
Thinking output <Think> <Sep> c </Think> <Ans> <1> <EOS>
Non-thinking output <Ans> <1> <EOS>
B. Repeated occurrences of one character (N = 4)
Query <BOS> <CountChar> D c S <Sep>
Shuffled input excerpt . . . aeSotlcrh . . . wce . . . stche . . .
Target positions 75, 79, 164, 178
Counts by character D: 0, c: 3, S: 1
Thinking output <Think> <Sep> S <Sep> c <Sep> c <Sep> c </Think> <Ans> <4> <EOS>
Non-thinking output <Ans> <4> <EOS>
C. Adjacent target occurrences (N = 7)
Query <BOS> <CountChar> b w k <Sep>
Shuffled input excerpt . . . Uhwc . . . pwde . . . e k\ne . . . aIkca . . . aewda . . . htwbgv
Target positions 12, 18, 174, 181, 207, 253, 254
Counts by character b: 1, w: 4, k: 2
Thinking output <Think> <Sep> w <Sep> w <Sep> k <Sep> k <Sep> w <Sep> w <Sep> b
</Think> <Ans> <7> <EOS>
Non-thinking output <Ans> <7> <EOS>
Architecture and optimization. We train one decoder-only Transformer from scratch for each
output format, using the same architecture and training settings (Table 5). No representation-
learning objective or scheduled sampling is used.
34
Table 5: Synthetic training and evaluation settings. Both modes use the same settings unless
the output format or loss component is specified. There is one training run per mode. Learning-rate
values refer to one-based optimizer steps.
Setting Value
Model and data
Transformer depth / heads per layer 4 / 8
Hidden / head dimensions 512 / 64 (approximately 12.7M parameters)
Feed-forward network Width 2,048; GELU with tanh approximation
Normalization / dropout Pre-LayerNorm / 0 throughout the model
Position encoding / capacity RoPE, base 10,000 / 384 token positions
Embedding sharing Input and output embeddings tied; the ten atomic count-output
vectors are untied
Input / query / count range 256 shuffled characters / 3 target characters / 1–10
Target-set pool / sampling seed 100 sets / 21,234
Training / validation / test allocation 80/10/10, with 255-character guard intervals
Optimization
Optimizer AdamW; β1 = 0.9, β2 = 0.999, ϵ = 10−8
Weight decay 0.01, applied to all model parameters
Gradient clipping Global ℓ2 norm capped at 1.0 before each optimizer step
Batch size 128 examples per optimizer step; no gradient accumulation
Training budget 10,000 optimizer steps; 1,280,000 sampled examples per mode,
including repeats
Precision bfloat16 autocast; model parameters remain in float32
Training seed 1234 for each independently trained mode
Learning-rate schedule
Peak learning rate ηmax = 3 × 10−4 at step 500
Linear warmup Steps 1–500; η1 = 6 × 10−7, rising linearly to ηmax
Cosine decay Steps 501–10,000; minimum learning rate η10,000 = 0
Loss-switch behavior Schedule continues at step 1,501; no restart or second warmup
Objectives and evaluation
Steps 1–1,500 Teacher-forced next-token cross-entropy over the full sequence
Steps 1,501–10,000 Task-output loss with count / marker / structure weights 8 / 8 /
16; Non-thinking has no marker term
Task-output loss reduction Per-example mean within each component, then the weighted sum
and batch mean (Eq. 6)
Selection / evaluation inputs 200 / 100; respectively 20 / 10 per count
Analysis checkpoints Steps 0, 100, 200, . . . , 10,000 (101 checkpoints)
Training objectives. For steps 1–1,500, we minimize next-token cross-entropy over all non-
padding targets. From step 1,501 onward, the loss includes task-output targets only, beginning with
<Ans> for Non-thinking and <Think> for thinking. Let ¯ℓC , ¯ℓR, and ¯ℓS denote cross-entropy averaged
first within each example over final count tokens, retrieved-character tokens, and structural tokens,
respectively, and then across the batch. The objectives are
LNT = 8¯ℓC + 16¯ℓS , LT = 8¯ℓC + 8¯ℓR + 16¯ℓS . (6)
For thinking, structural tokens include <Think>, every <Sep>, </Think>, <Ans>, and <EOS>; for
Non-thinking they are <Ans> and <EOS>. Separately averaging the components keeps the final count
35
coefficient independent of trace length.
Tiny Shakespeare is a small corpus, approximately 1 MB, and the original nanoGPT configura-
tion explicitly anticipates overfitting (Karpathy, 2022). To monitor generalization, Fig. 17 reports
full-sequence cross-entropy on inputs from the training and validation regions. We retain this eval-
uation loss after training switches to the weighted task-output loss in Eq. 6 at step 1,501, so the
plotted values remain comparable across training stages. The two curves largely overlap and do not
identify a clear onset of overfitting. The objective switch at step 1,501 is a preset training choice.0 5k 10k
Training step
5
10
15
20
Cross-entropy
A. Non-thinking loss
0 5k 10k
Training step
4
6
8
Cross-entropy
B. Thinking loss
1 2 3 4 5 6 7 8 9 10
True count
0
25
50
75
100
Accuracy (%)
C. Answer accuracy
Non-thinking Thinking Training region Validation region
Figure 17: Training and counting behavior. A/B: full-sequence, token-weighted cross-entropy
on evaluation inputs generated from the training (solid) and validation (dashed) regions of the
original corpus. Validation-region inputs are excluded from parameter updates. The dotted line
marks the objective change at step 1,500; this evaluation metric remains fixed. C: final-checkpoint
answer accuracy, with ten evaluation inputs per count and mode. Missing numeric answers are
incorrect.
Evaluation protocol. Unless stated otherwise, mechanistic analyses use disjoint selection and
evaluation sets from the held-out test region: 200 and 100 inputs, organized into 20 and 10 analysis
blocks, respectively, with one input per count N = 1, . . . , 10. The sets share neither input identities
nor (target-set, source-window-start) pairs. Head rankings and representation transforms are fitted
on selection inputs. Answer accuracy uses greedy generation, counting missing or incorrect answers
as failures. Attention and representation measurements use teacher-forced prefixes; final-answer
prompt and trace ablations use each model’s generated prefix.
G.2 Broad and targeted retrieval heads
Broad and targeted retrieval. Let Ah(q, p) be the attention weight from query position q to
source position p in head h, and let qA be the <Ans> position whose logits predict the final count.
Let sk be the position of input character xpk in the complete token sequence, including the query
prefix; pk remains its index within x. For one input, define total target attention Mh, its normalized
distribution πhk over the target occurrences, and the corresponding entropy Hh by
Mh =
N∑
k=1
Ah(qA, sk), πhk = Ah(qA, sk)
Mh
, Hh = −
N∑
k=1
πhk log πhk. (7)
36
The broad score is Bh = Mh exp(Hh)/N . We set Bh = 0 if Mh = 0 and use 0 log 0 = 0. The
factor exp(Hh) is the effective number of attended target occurrences: uniform target attention
gives Bh = Mh, while concentrating the same mass on one occurrence gives Bh = Mh/N . Thus,
the score rewards both mass and coverage.
For thinking, qk is the <Sep> query immediately before the kth trace character. The targeted
score is
Th = 1
N
N∑
k=1
Ah(qk, sk). (8)
This score distinguishes the corresponding occurrence from other instances of the same character.
Each score is computed within an input and then averaged equally across inputs. Heads are ranked
globally across all four layers; LℓHj denotes layer ℓ and head j, both one-based.H1 H2 H3 H4 H5 H6 H7 H8
Head
L1
L2
L3
L4
Layer
A. Non-thinking: broad
0.000 0.025 0.050
Broad score Bh
H1 H2 H3 H4 H5 H6 H7 H8
Head
L1
L2
L3
L4
Layer
B. Thinking: targeted
0.0 0.5 1.0
Targeted score Th
Figure 18: Retrieval-head scores. A: Non-thinking broad score Bh at the final-answer query. B:
thinking targeted score Th at trace retrieval queries. Each cell shows one head’s score at step 10,000,
averaged equally over 100 teacher-forced evaluation inputs. Rows are layers L1–L4; columns are
heads H1–H8. The panels use separate color scales, matching Fig. 24, with no normalization across
heads.
Head bank ablation. We zero selected head outputs before the attention output projection,
from the final-answer query (Non-thinking) or final marker query (thinking) through EOS, capped
at 64 new tokens. We measure final count accuracy for Top-1–4 broad heads on all 100 Non-
thinking inputs, and next-marker accuracy for Top-1–8 targeted heads on 88 thinking inputs. The
latter have N ≥ 2 and an available clean final retrieval query; their selection ignores final count
correctness. No inputs are excluded based on intervened outputs.
A marker denotes a target-character token. For thinking, we intervene at the N th <Sep> in
the clean generated trace and score whether the next token equals aN ; non-character outputs are
errors.
Controls match the number of heads per layer. We enumerate all feasible sets, using the least
possible overlap with selected heads; Top-4 Non-thinking controls share one head. Non-thinking
controls also preserve L1H3, following a diagnostic in which its ablation made all 100 inputs repeat
<Ans>. Replacing its values with the fixed value vector for the non-target character o restored
37
every clean first-token prediction, suggesting an approximately constant contribution to answer-
token generation.
In Fig. 19, Non-thinking Top-4 ablation reduces final count accuracy to 7%, versus a 15% control
mean. Thinking next-marker accuracy is 85.2% versus 93.2% at Top-4, and 68.2% versus 77.3% at
Top-8. These ablations support the selected heads’ roles in final count prediction and local marker
retrieval, respectively.1 2 3 4
Ablated heads
0
10
20
30
40
Accuracy (%)
A. Non-thinking: final count
1 2 3 4 5 6 7 8
Ablated heads
60
70
80
90
100
Accuracy (%)
B. Thinking: next marker
Broad heads Targeted heads Control mean (range) Clean
Figure 19: Retrieval head ablation. A: final count accuracy on all 100 Non-thinking inputs, for
Top-1–4 broad heads. B: next-marker accuracy on 88 eligible thinking inputs, for Top-1–8 targeted
heads. Lines show selected sets, control means, and clean baselines; shading spans the control sets.
The axes each span 40 percentage points; B is truncated to 60–100%.
G.3 Count representations and causal interventions
Counter states and answer states. Following the main-text terminology, counter states rep-
resent counting progress at prompt or trace items, and answer states support the final count pre-
diction at the answer query. We decode running index k from residual states at prompt position
sk (Non-thinking) or the trace-character token ak (thinking), and final count N from the answer-
query state at qA. Here k counts target occurrences encountered in the prompt or emitted in the
trace, respectively. States are taken after each Transformer block, before final normalization, using
teacher-forced prefixes. Each mode has 550 occurrence states and 100 answer states from ten inputs
per count.
Each thinking occurrence adds two trace tokens, so running index covaries with trace length
and position. Counter-state analyses therefore retain these structural cues alongside item content.
PCA visualization. All four PCA panels use the layers selected by discovery NCC: L2/L4
for Non-thinking/Thinking running indices and L4/L2 for their final counts (Fig. 20). Selection
searches the four Transformer blocks and uses the grouped-validation rule below. A separate
three-component PCA is fitted for each mode and endpoint. Selection-set standardization and
PCA are applied unchanged to evaluation states, without whitening. Coordinates are not directly
comparable across these independent projections.
38
0
25 −25
0
−25
0
25
0
20 −20
0
20
−20
0
20
−25
0 −25
0
25
−25
0
25
0
20 −20
0
−20
0
20
1 10
A. Non-thinking: running index (L2) B. Thinking: running index (L4)
C. Non-thinking: final count (L4) D. Thinking: final count (L2)
Running index / final count
PC1 PC2
PC3
PC1 PC2
PC3
PC1 PC2
PC3
PC1 PC2
PC3Figure 20: Count geometry. Discovery NCC selects L2/L4/L4/L2 for A/B/C/D. Separate PCA
projections show 550 running-index states (A/B) and 100 answer states (C/D) per mode. Outlined
class means are connected in label order. The three components explain 50.9/48.1/74.0/71.7% of
selection variance in A/B/C/D. All panels use the same camera view and equal coordinate units
within each panel.
Nearest-centroid decoding. For quantitative comparison, we standardize states and apply
whitened 16-component PCA. A nearest-centroid classifier (NCC) assigns each transformed state
z to the closest class centroid μc:̂
y(z) = arg min
c∈{1,...,10}
∥z − μc∥2
2, BA = 1
10
10∑
c=1
1
nc
∑
i:yi=c
1{̂y(zi) = c}. (9)
Here nc is the number of evaluation states in class c. Balanced accuracy weights all ten labels equally
(chance: 10%), accounting for the greater frequency of smaller running indices. The transform
and centroids are fitted only on selection states. Marked layers maximize five-fold NCC balanced
39
accuracy on the selection set, keeping each input block together; ties use logistic balanced accuracy
and then earlier layers. Every fold fits its preprocessing and classifiers using training inputs only.
At the NCC-selected layers, final count decoding reaches 99% for Thinking (L2) and 24% for
Non-thinking (L4). Thinking running-index accuracy ranges from 15% to 34% across Transformer
blocks (Fig. 21). Thus, Thinking separation is strongest at the final answer; decoding alone does
not establish that the model uses this information.1 2 3 4
Post-block layer
0
25
50
75
100
Balanced accuracy (%) A. Running index
1 2 3 4
Post-block layer
0
25
50
75
100
Balanced accuracy (%) B. Final count
Non-thinking Thinking Chance (10%)
Figure 21: Count decoding across layers. Balanced NCC accuracy for running index (A)
and final count (B), using teacher-forced states. Squares mark layers selected by grouped cross-
validation. Preprocessing and centroids are fitted only on selection inputs.
Sources of the next marker. At the query for k = max(1, ⌊N/2⌋) under teacher forcing, we
zero states at the selected prompt or trace positions at the embedding output and after every block,
preserving token positions. We separately ablate prompt targets, the latest completed trace item,
or the full preceding trace; controls ablate an equal number of non-target prompt positions. Next-
marker accuracy falls from 96% to 21% after prompt-target ablation and to 79% after either trace
ablation (Fig. 22). All 100 inputs remain in the evaluation, including 30 with no completed trace
item. The next marker is therefore sensitive to both prompt targets and available trace history.Prompt: ... a ... b ... a ...
Trace: <Sep> a <Sep> b
Next marker: ?
Token positions are unchanged
A. Ablation positions
Prompt
targets
Recent
trace item
Full trace
history
0
25
50
75
100
Accuracy (%)
21
79 79
95 96 96
B. Next-marker prediction
Clean (96%) Prompt/trace ablation Control ablation
Figure 22: Sources of the next marker. A: prompt and trace schematic. B: next-marker
accuracy after prompt or trace ablation, with controls at non-target prompt positions. All 100
inputs are retained, including 30 without prior trace items.
40
Counter-state transplantation. We copy the full separator and character states of source trace
item d into target trace item k = d ± 1, then continue generation without further patching. The
order of target characters, the total count, and the target run’s visible prefix remain fixed. Adding or
removing two non-target characters from the source prompt aligns the transplanted token positions.
On 20 selection inputs (N = 10, d = 6), we select L1 from L1–L3: require positive median
shifts in the logit difference between the source and target continuations in both directions, then
take the earliest layer reaching 95% of the peak median input-averaged shift. Evaluation uses
ten separate N = 10 inputs at d ∈ {4, 6, 8}. For each length h = 1, . . . , 4, we compare the
first h generated characters with the source continuation (ad+1, . . . , ad+h). A pair is eligible if
both continuations have at least h characters and the source sequence differs from the target
continuation (ak+1, . . . , ak+h). Eight of the ten inputs contribute eligible pairs at each length.
We average exact matches within input, then across eligible inputs; short or malformed outputs
fail. Source-continuation exact match is 45.0% for one character and 16.7% for four characters
(Fig. 23A). Wide intervals and different eligible pair sets across lengths limit conclusions about
sustained continuation.
Sources of the final answer. On all 100 inputs, each model generates its prefix through <Ans>.
We repeat the prompt and trace ablation protocol above at the final count query, targeting prompt
occurrences or generated trace positions. Thinking accuracy falls from 95% to 59% after trace
ablation and remains 95% after prompt-target ablation (Fig. 23B). Together, these prompt and
trace ablations support prompt-based character retrieval and trace-based final count readout.
Answer-state transplants. At each layer, we transplant the full answer-query state using
teacher-forced prefixes and 180 directed pairs of adjacent counts within evaluation blocks. We
score agreement with the source run’s clean prediction. Before patching, this compares the clean
target and source predictions: thinking correctly predicts their distinct counts, giving 0% agree-
ment; Non-thinking gives the same prediction on 36 of 180 pairs, giving 20%. All clean source
predictions are valid count tokens.
At L3, with one block remaining, agreement rises from 20% to 75% for Non-thinking and from
0% to 100% for thinking (Fig. 23C). Both reach 100% at L4, where the copied state directly feeds
final normalization and the output projection. Non-thinking matches the source prompt’s true
count on only 17.2% of these pairs, reflecting errors in the source predictions.
41
1 2 3 4
Subsequent markers
0
25
50
75
100
Exact match (%)
45.0 39.4
21.9 16.7
A. Source continuation
Prompt
targets
Generated
trace
0
25
50
75
100
Answer accuracy (%) 95
59
95 95
B. Final-answer sources
1 2 3 4
Patching layer
0
25
50
75
100
Match (%)
C. Source prediction
Source state
Clean (95%)
Prompt/trace ablation
Control ablation
Non-thinking
Thinking
After patching
Before patchingFigure 23: Trace continuation and final-answer interventions. A: input-averaged source-
continuation exact match after an L1 item transplant, with eight inputs and 26/30/26/20 pairs for
lengths 1/2/3/4. Error bars: 95% percentile intervals from 10,000 input-bootstrap resamples. B:
thinking answer accuracy after prompt or trace ablation on 100 generated prefixes. Controls ablate
equally many non-target prompt positions; the dotted line marks clean accuracy. C: agreement
with the source run’s clean prediction on 180 pairs using teacher-forced prefixes.
G.4 Learning dynamics of retrieval and counting
Attention roles and successor-like heads. We track all 32 heads every 100 steps from initial-
ization, using the same 100 teacher-forced evaluation inputs (Fig. 24A–D). Alongside broad and
targeted retrieval, we measure successor-like attention from each trace character at rk = qk + 1 to
its preceding separator at qk:
Uh = 1
N
N∑
k=1
Ah(rk, qk). (10)
Scores are averaged equally across inputs. Non-thinking develops broad retrieval in shallow layers,
while thinking develops targeted retrieval in deeper layers. Local successor-like attention strength-
ens earlier: at step 400, the largest Uh across thinking heads is 0.267, while the largest Th is
0.006.
Gould et al. (2024) identify successor heads whose outputs promote the next member of an
ordered sequence, such as numbers or days of the week. Our term successor-like describes the
local attention pattern in Uh, without assuming this increment function. The preceding separator
is the query used to retrieve the current character; attending back to it may carry retrieval-query
information forward to the completed item’s state.
At the final checkpoint, L2H4 has the highest Uh on the 200 selection inputs. In a separate assay
on 100 evaluation inputs, we zero its output at generated trace-character positions immediately
following <Sep>. This position-restricted intervention differs from the sustained retrieval-head
ablations above. Final count accuracy falls from 95% to 45%, versus 79–94% for three same-layer
controls (L2H1, L2H5, and L2H8). Exact-trace accuracy falls from 87% to 39%, with all outputs
remaining valid in format. These results support L2H4’s contribution to trace processing and
counting behavior.
42
0 5k 10k
L1H1
L1H5
L2H1
L2H5
L3H1
L3H5
L4H1
L4H5
A. Non-thinking
Broad
0 5k 10k
B. Thinking
Broad
0 5k 10k
C. Thinking
Targeted
0 5k 10k
D. Thinking
Successor-like
0.000 0.025 0.050
Broad score
0.0 0.5 1.0
Targeted / successor-like score
0 5k 10k
Training step
0
25
50
75
100
Balanced accuracy (%) E. Running index
0 5k 10k
Training step
0
25
50
75
100
Balanced accuracy (%) F. Final count
Training step
Non-thinking (L2) Thinking (L4) Non-thinking (L4) Thinking (L2)Figure 24: Attention and count decoding during training. All panels use a linear training-
step axis and the same 100 evaluation inputs. A–D: attention scores for all 32 heads across 101
checkpoints; rows retain head identity and white lines separate layers. A/B share the broad-score
scale; C/D use a fixed 0–1 scale for targeted and successor-like attention. E/F: balanced NCC
accuracy for running index and final count at eleven checkpoints. Layers are selected by final-
checkpoint discovery NCC and remain fixed; transforms and centroids are fitted on selection states
at each checkpoint. Vertical dotted lines mark the objective switch at step 1,500; horizontal dotted
lines in E/F mark 10% chance accuracy.
Decoding and generation. We evaluate NCC at steps 0, 100, 200, 400, 800, 1500, 2500, 4000,
6000, 8000, 10000 (Fig. 24E/F). Layers remain fixed at the final-checkpoint discovery NCC selec-
tions: L2/L4 for Non-thinking/Thinking running indices and L4/L2 for their final counts. The
grouped cross-validation rule and tie-breaks are the same as in Fig. 21; PCA displays use these
same layers. Earlier checkpoints do not reselect layers. Transforms and centroids are refitted on
selection states at each checkpoint.
At step 400, thinking final count decoding reaches 100% with a correct teacher-forced trace,
while free-generation count accuracy is 12% and exact-trace accuracy is 2%. Thus, the final count
becomes readable given a correct trace before the model can reliably generate that trace. Interme-
43
diate running index decoding follows a different trajectory, falling from 73.7% at step 200 to 31.4%
at the final checkpoint. Early decoding may reflect regular trace structure before accurate retrieval
develops. Successor-like attention is still weak at step 200 (maximum Uh = 0.025), so its role in
this peak remains unverified.
G.5 Relation to the main experiments
[TODO: Append after finishing the body part.]
Retrieval mechanisms. Head-score maps and ablations support the main distinction between
broad aggregation in Non-thinking and targeted retrieval in thinking (Figs. 18 and 19). The thinking
ablation specifically tests local next-marker retrieval.
[GPT] Counter-state continuation and answer readout. Prompt and trace ablations sup-
port prompt-based retrieval and trace-based final answering (Figs. 22 and 23B). [GPT] Counter-
state transplants shift trace continuation, while late answer-state transplants support final count
readout in both modes (Fig. 23A/C).
H Further details for additional tasks
We extend the counting experiments to retrieval of the kth record and counting within a specified
category, measuring final-answer accuracy and testing heads selected separately for each task.
H.1 Experimental design
Tasks and inputs. Each passage contains ten records rj = (ej , vj , cj ) in passage order, with
entity ej , numeric score vj , and category cj . The retrieval task asks for (ek, vk), varying k = 1, . . . , 10
on the same city-record passage within each seed. Category counting asks for Nc = ∑10
j=1 1{cj = c}.
Each seed supplies five passages with 1, 3, 5, 7, or 9 city records and the remaining records assigned
to flowers; both categories are queried on every passage. For example, a passage with three city
records has city and flower counts of 3 and 7. This construction preserves the main experiment’s
background, record order, scores, and passage wrapper, changing only the category word and entity
name where needed.
Models and generation. We evaluate Qwen3-8B and Gemma4-E4B without additional training,
using bfloat16 weights, SDPA generation, and greedy decoding. Non-thinking permits 64 new
tokens; Thinking permits 4,096, with reasoning enabled and no forced enumeration or first-list
cutoff. Each task contains 300 inputs from 30 seeds: 200 discovery inputs (seeds 1234–1253) and
100 evaluation inputs (1254–1263). Inputs are shared across models and modes, giving 2,400 natural
outputs. Prompts contain approximately 10,000 tokens. Only discovery inputs determine the head
rankings.
As in Appendix C.1, each task has a complete user-message template and two response-instruction
variants. Replace {passage} with the experimental passage and {response_instruction} with
the chosen mode’s block. Box titles and role labels are annotations; angle-bracketed output place-
holders are literal.
44
Retrieval of the kth record. Set {k} to the requested position (1, . . . , 10). Non-thinking uses
the Needle: assistant prefill after chat-template rendering; Thinking uses no prefill.
Prompt | Retrieval of the kth record: user template
User message
You will need to find a specified city-score audit record in passage order.
A city-score audit record names one city and gives that city’s numeric score.
<passage>
{passage}
</passage>
Which city-score audit record is number {k} in passage order?
Count occurrences from the beginning of the passage, starting at 1.
Return the actual city name and numeric score of that record.
{response_instruction}
Prompt | Retrieval of the kth record: response instructions
Non-thinking
Do not explain, reason aloud, quote, or list any records.
Use no spaces around the colon or vertical bar.
Your entire response must be exactly one line:
Needle:<city>|<integer>
Thinking
Reason concisely without repeating or restarting.
Stop as soon as you identify that record, then output exactly one line:
Needle:<city>|<integer>
Counting a specified category. Set {category} to city or flower. Non-thinking uses the
Total: assistant prefill after chat-template rendering; Thinking uses no prefill.
45
Prompt | Category counting: user template
User message
You will need to count only {category}-score audit records in the passage below.
A city-score audit record names one city and gives its numeric score.
A flower-score audit record names one flower and gives its numeric score.
<passage>
{passage}
</passage>
How many {category}-score audit records are in the passage?
Count only matching audit records. Ignore audit records of the other category and
ordinary passage text.
{response_instruction}
Prompt | Category counting: response instructions
Non-thinking
Do not explain, reason aloud, quote, or list any records.
Write the count using ordinary decimal digits, with no space after the colon.
Your entire response must be exactly one line:
Total:<integer>
Thinking
Reason concisely without repeating or restarting.
Stop as soon as you determine the count, then output exactly one line:
Total:<integer>
For Non-thinking, we prepend the saved answer prefix and remove end tokens. For Thinking, we
separate reasoning from the final response using </think> for Qwen and <channel|> for Gemma,
then remove supported response wrappers and end tokens; already-separated final responses are
also accepted. The entire final response must match Needle:<city>|<digits> or Total:<digits>;
surrounding whitespace and whitespace after separators are allowed. City names are trimmed and
matched case-sensitively, and digit strings are compared as integers. Extra prose, missing fields, or
a detected but unclosed reasoning channel yield an unparsed answer and count as errors. Capped
outputs remain in the denominator and follow the same rule.
Here we average accuracy within data-generation seeds, then equally across seeds (30 for natural
behavior; ten for interventions). We report 95% percentile intervals from 20,000 bootstrap resamples
of seeds, paired across conditions for intervention contrasts.
H.2 Behavioral comparison between the two modes
Thinking achieves higher final-answer accuracy for both models on both tasks (Table 6). Across re-
quested positions and category counts, Qwen’s Thinking accuracy remains high, whereas Gemma’s
generally declines at later positions and larger counts (Fig. 25).
46
Table 6: Natural final-answer accuracy (%). Each condition includes all 300 inputs from 30
seeds. Brackets give 95% confidence intervals (CIs).
Task Model Non-thinking Thinking
Kth record Qwen 13.00 [11.33, 15.00] 97.67 [94.67, 100.00]
Kth record Gemma 26.33 [23.00, 29.67] 78.00 [70.00, 85.67]
Category count Qwen 32.33 [28.33, 36.33] 96.00 [93.67, 98.33]
Category count Gemma 30.33 [27.00, 34.00] 61.67 [54.67, 68.67]1 2 3 4 5 6 7 8 9 10
Requested position k
0
25
50
75
100
Answer accuracy (%)
A. Kth record
1 3 5 7 9
Target-category count
0
25
50
75
100
Answer accuracy (%)
B. Category count
Qwen3 / Non-thinking
Qwen3 / Thinking
Gemma4 / Non-thinking
Gemma4 / Thinking
Figure 25: Final-answer accuracy by position and category count. A: requested record
position (30 inputs per point). B: true target-category count, pooling city and flower questions
(60 per point). Blue denotes Qwen and orange Gemma; solid circles denote Thinking and dashed
squares Non-thinking. Aggregate 95% CIs appear in Table 6.
Gemma’s Thinking results include 12 unparsed retrieval answers and 16 unparsed category
answers, with one retrieval output reaching the token limit. All other conditions have no unparsed
or capped outputs. These comparisons include each mode’s instructions and generation budget.
H.3 Retrieval-head distributions and causal tests
We next test whether task-specific retrieval heads contribute to these behaviors. Broad-head inter-
ventions measure Non-thinking final-answer accuracy; targeted-head interventions measure next-
entity accuracy during Thinking. Head discovery and intervention evaluation use disjoint inputs.
Head identification and parsing. For targeted retrieval, we first parse the reasoning channel
by matching input city and flower names case-insensitively. A rank parser links mentions to local
numeric, ordinal, or running-count markers, splits at restarts from 1, and retains the longest con-
tiguous 1, . . . , M sequence (earliest on ties). Repeated entities are retained if their ranks advance. A
structural parser recognizes terminated numbered, bulleted, ordinal, or supported record-sentence
lists; its sequence replaces a rank sequence only by extending the exact entity prefix, or is used when
47
no rank sequence exists. If both fail, we order the first mention of each distinct entity whose regis-
tered score occurs within the next 96 characters. These inferred positions index mentions without
establishing count updates. Neither the requested answer nor final-answer correctness determines
the selected sequence.
From consecutive parsed records, we register the middle eligible transition (the earlier of two
middle transitions). For Qwen, its query q∗ follows a marker preceding the next entity when
available; otherwise, and for Gemma, it follows the preceding item’s semantic endpoint (P0). We
advance to the first compatible original-token boundary through whitespace or punctuation, re-
maining before the next entity, and retain the original generation tokens. The targeted score in
Eq. (2) uses this single query and the full input-record span S∗ of the next parsed entity. This
entity can differ from the requested kth record or belong to either category. Broad retrieval instead
applies Eq. (1) at the Non-thinking final-answer query qA over all J = 10 complete input-record
spans. Its implementation uses phj = mhj /(Mh + ϵ) and log(phj + ϵ), with ϵ = 10−12 and Bh = 0
for Mh ≤ ϵ.
We rank heads across all layers by their discovery means within each task, model, and scoring
condition, breaking ties by layer and head index (Fig. 26). Broad retrieval uses all inputs in each
split. Targeted retrieval requires an aligned transition: discovery/evaluation counts are 167/83 and
149/79 for Qwen on retrieval and category counting, and 190/94 and 180/90 for Gemma. Inputs
without a transition remain in the natural evaluation. Interventions include all ten evaluation seeds,
retain clean errors, and keep eligible inputs fixed across K.
Ablation protocol and evaluation. Selected ablation zeros the frozen Top-K heads’ output
slices before the attention output projection. Broad ablation acts only at qA in one prefix forward
pass, followed by at most 64 new tokens. Targeted ablation acts at q∗ and subsequent decoding
positions for at most 256 tokens. Clean uses the same prefixes and budgets.
For the targeted outcome, the continuation parser compares the earliest recognized entity with
the registered next entity, ignoring case. Recognition uses input names and generic record forms
(“received a score,” “with a score,” or name–score pairs), including city/flower audit forms that
allow unlisted names. An earlier wrong entity is an error even if the target appears later. If none is
recognized, a token fallback requires a saved target at continuation offset zero and a continuation
beginning with its complete original entity-token sequence. Only entity identity is scored.
Random accuracy is averaged over three control sets matching Selected’s head count per layer.
Heads are sampled without replacement from unselected heads whenever possible. Only broad kth-
record ablation at the largest K requires overlap: two heads in one layer per model and control set.
Qwen’s broad grid is K ∈ {1, 2, 4, 8, 16, 32, 64, 128} and its targeted grid is {32, 64, 80, 96, 112, 128};
Gemma uses {1, 2, 4, 6, 8} for both. As in the main experiment, we report the full scans of Selected
and Random accuracies.
48
1 16 32
1
13
25
36
Layer
A. Broad Bh
0 0.85
1 16 32
1
13
25
36
B. Targeted Th
0 0.65
1 16 32
1
13
25
36
C. Broad Bh
0 0.65
1 16 32
1
13
25
36
D. Targeted Th
0 0.4
1 4 8
Head
1
15
29
42
Layer
E. Broad Bh
0 0.65
1 4 8
Head
1
15
29
42
F. Targeted Th
0 0.25
1 4 8
Head
1
15
29
42
G. Broad Bh
0 0.3
1 4 8
Head
1
15
29
42
H. Targeted Th
0 0.15
Kth record Category count
Qwen3-8B
Gemma4-E4BFigure 26: Discovery scores for both additional tasks. Task groups pair broad (Bh, Non-
thinking) and targeted (Th, Thinking) scores; rows show Qwen (blue) and Gemma (orange). Cells
represent heads, with one-based layer and head indices. Each panel has an independent, unclipped
linear scale from zero to its labeled maximum; compare numerical scores using the colorbars.
Effects of head ablation. Task-ranked targeted heads contribute causally to next-entity gen-
eration in both additional tasks (Fig. 27A–D). Qwen’s Selected accuracy decreases monotonically
over the scanned K values, while Gemma shows a pronounced separation from Random at K = 6
and 8, with mixed effects at smaller K. At the largest tested K (128 for Qwen; 8 for Gemma),
Selected versus Random accuracy is 10.9% versus 98.1% (Qwen) and 44.7% versus 87.9% (Gemma)
for kth-record retrieval; for category counting, the corresponding accuracies are 16.5% versus 91.3%
and 17.6% versus 53.6%. The layer-matched controls show that the impairment exceeds the effect
of removing the same number of heads from the same layers.
Broad-head ablation also reduces final-answer accuracy at some K, but its separation from
Random is weaker and less consistent across the scan (Fig. 27E–H). Low Clean accuracy (13–29%)
leaves limited room for further declines. Additional ordering or category-selection demands may
introduce errors beyond retrieval, although their role in weakening the ablation effect remains
untested. Differences in outcomes, eligible inputs, and intervention duration preclude a direct
comparison of head importance between the two assays.
49
32 64 80 96 112 128
0
50
100
A. Targeted: kth record
1 2 4 6 8
0
50
100
B. Targeted: kth record
32 64 80 96 112 128
0
50
100
C. Targeted: category count
1 2 4 6 8
0
50
100
D. Targeted: category count
1 2 4 8 16 32 64 128
0
20
40
E. Broad: kth record
1 2 4 6 8
0
20
40
F. Broad: kth record
1 2 4 8 16 32 64 128
Ablated heads K
0
20
40
G. Broad: category count
1 2 4 6 8
Ablated heads K
0
20
40
H. Broad: category count
Qwen3-8B Gemma4-E4B
Next-entity accuracy (%)Final-answer accuracy (%)
Selected ablation Random control 95% CIFigure 27: Top-K head ablation. Absolute accuracies for Selected (solid circles) and Random
(dashed open squares; mean of three banks). A–D: Thinking targeted ablation, measuring next-
entity accuracy. E–H: Non-thinking broad ablation, measuring final-answer accuracy. Columns
show Qwen (blue) and Gemma (orange); rows separate tasks. Shading shows pointwise 95% CIs.
Qwen’s broad axes are logarithmic. Clean accuracies for Qwen/Gemma are 100.00/97.00% for kth-
record retrieval and 94.78/69.36% for category counting in the targeted assay; the corresponding
broad-assay accuracies are 13.00/26.00% and 25.00/29.00%.
H.4 Implications for the retrieval mechanisms
[TODO: Claim that these tasks extend the Thinking advantage and support targeted
retrieval during local next-entity generation.]
50

==> sections/intro_v1.tex <==
\section{Introduction}

%CoT changes both the amount of computation available to a language model and the sequence of tokens through which that computation is expressed. These two effects are difficult to separate in unconstrained reasoning tasks. Long-context counting provides a useful test bed because success requires two identifiable operations: retrieving all relevant records from a long passage and aggregating them into an exact integer. The same task can be solved either in one final answer state or by writing a multi-step trace, making it possible to ask whether CoT changes the underlying information-flow strategy. \YZ{This is written by ChatGPT, right?}\LS{Yes, just put some rundom things here.}

%Recent few years have seen internal mechanisms
%In the recent few years, interpretability research of large language models (LLMs) has enriched our understanding of LLMs 

Long-context reasoning has become a pillar of large language models (LLMs) in solving complex tasks, where models generate a sequence of chain-of-thought (CoT) tokens before reaching a final answer. Yet, existing interpretability research mostly focuses on short input prompts and model generation includes no long CoT traces. A critical gap exists between the ever-growing inference-time scaling and our limited understanding of model's internal mechanism.

To understand long-context inference and CoT reasoning, we present a case study on \textit{long-context counting} partly based on needle-in-a-haystack (NIAH)  benchmarks \cite{} \YZ{cite RULER, etc}. In a nutshell, this task asks the model to count the number of records (or needles, denoted by $N_1,N_2,N_3,\ldots$) inserted in a long passage (haystack). For example, the following input prompt contains two audit records followed by a query
\begin{center}
\small
``\texttt{<passage>} $\ldots$ \textit{In the 2024 city score audit, Paris received a score of 92.} $\ldots$
\textit{In the 2024 city score audit, Vienna received a score of 73.} $\ldots$ \texttt{</passage>}\\
How many city-score audit records are in the passage?''
\end{center}
A non-reasoning model typically emits a final-answer count such as ``Total: 8'', while a reasoning model (often with the Thinking mode on) generates a CoT trace enclosed in the <think></think> tag before the final-answer count. \YZ{Do we need to explain this? I think we need to explain what CoT means, since direct enumeration is related by different.} 

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{figures/main_figure_v4.pdf}
    \caption{%\textbf{Mechanism and representation comparison of two modes.}
    \textbf{Two retrieval mechanisms and contrasting representations.}
    \textbf{A.} Non-thinking distributes final-query attention across prompt needles. \textbf{B.} Thinking targets successive needles as its trace progresses. \textbf{C.} PCA projections of needle end representations, colored by running count-index, with numbered centroids. Held-out nearest-centroid accuracy is 46\% for Non-thinking and 98\% for Thinking. Attention and representations are based on Qwen3-8B with 20K-token inputs.
    %Construction and interpretation are detailed in Appendix~\ref{app:figure-details}.
    }
    \label{fig:main}
\end{figure}

Long contexts and CoT reasoning bring new challenges to mechanistic analysis, leaving existing insights from in-context learning and steering \YZ{find related work? Find retrieval work (RAG, NIAH), or CoT analysis.} insufficient. First, long contexts require models to locate relevant information while they are generally brittle to growing contexts \YZ{cite lost-in-the-middle paper, find more empirical papers about long-context issues}, yet we have limited understanding about such brittleness. Second, common heuristics attribute the benefits of CoT to step-by-step decomposition at inference time, yet realistic long-context reasoning behaviors are much involved than theory and in toy settings \cite{}. In essence, CoT amounts to a dynamic procedure: Starting from an input prompt, a model emits tokens one by one, which iteratively grows the context. \YZ{what's the status quo about this dynamic heuristic?}

%Common heuristics attribute the benefits of CoT reasoning to the step-by-step decomposition of a complex task at inference time. \YZ{summarize the current understanding of CoT reasoning and limitations.} While the benefits are evident in theory and in toy settings \cite{}, realistic long-context reasoning behaviors are much less explored, leaving the internal mechanism of reasoning poorly understood. Compared with existing interpretability research on in-context learning and steering \cite{}, CoT brings new challenges due to its dynamic procedure: Starting from an input prompt, a model emits tokens one by one, which iteratively grows the context.

%implicit reasoning vs.~explicit reasoning

Fundamental questions pretraining to reasoning appear: \textit{Do reasoning models develop specialized attention and better representations? What information is retained over the long growing context?} \YZ{search for signal-processing and information theory papers} We address these questions using the counting task as a clean case study: counting is a well-defined mapping from the context to an integer. This allows mechanism-level analysis to evaluate whether the models maintain sufficient internal count-state over the reasoning trace.

Our key finding is that two distinct mechanisms govern non-reasoning and reasoning modes (Figure~\ref{fig:main}). The former depends on \textbf{broad retrieval}, where the model attends to all prompt needles at the answer token. However, broad retrieval is unreliable at high counts or long contexts, producing noisy count-encoding representation. In contrast, the latter depends on \textbf{targeted retrieval}, where the model attends to needles one by one and  enumerates relevant needles in CoT traces. During reasoning process, the model forms compact representations, which maintain and update an count state, even in the absence of explicit numbering. 

%Do reasoning models maintain and update approximately sufficient internal states?

Below, we summarize our main contributions. %to non-reasoning and reasoning.

\begin{enumerate}
    \item \textbf{A comprehensive comparison across model families.} %Evaluating model performance for long-context counting 
    Across needle counts, prompt length, and model families, we find that needle counts and context lengths deteriorate model accuracy for non-reasoning models much more than reasoning models. (Sec.~\ref{sec:cross-model})
    %We evaluate model performance for our long-context task under varying needle counts (1--20) and prompt length (1K--20K tokens) across ?? models.
    \item \textbf{A mechanistic contrast between the two modes.} Non-reasoning models broadly attend to all prompt needles, collecting noisy representations at lower layers. In contrast, reasoning models target needles one by one in CoT traces, forming compact representations (Sec.~\ref{sec:non-thinking}--\ref{sec:thinking})
    \item \textbf{A controlled synthetic experiment on the emergence and specialization of attention.} A small transformer trained from scratch for counting produces broad retrieval; with CoT traces provided during the same autoregressive training, targeted retrieval emerges. (Sec.~\ref{sec:emergence})
\end{enumerate}

%\append{Figure: A main figure with multiple comparison, including prompt demo, attention mass heatmap, and PCA count manifold demonstration.}

==> sections/intro_v2.tex <==
\section{Introduction}\label{sec:intro}

Long-context reasoning has become a pillar of large language models (LLMs) in solving complex tasks, where models generate a sequence of Chain-of-Thought (CoT) tokens before reaching a final answer. Yet, existing interpretability research mostly focuses on short input prompts and output generation without long CoT traces. A critical gap exists between the ever-growing inference-time scaling and our limited understanding of models' internal mechanisms.

To understand long-context inference and CoT reasoning, we present a case study on \textit{long-context counting} partly based on needle-in-a-haystack (NIAH) benchmarks
\citep{kamradt2023needle, hsieh2024ruler}. In a nutshell, this task asks the model to count the number of records (or needles, denoted by $N_1,N_2,N_3,\ldots$) inserted in a long passage (haystack) like Paul Graham essays. For example, the following input prompt contains two audit records followed by a query:
\par\begingroup\centering
``\texttt{<passage>} $\ldots$ \textit{In the 2024 city score audit, Paris received a score of 92.} $\ldots$
\textit{In the 2024 city score audit, Vienna received a score of 73.} $\ldots$ \texttt{</passage>}\\
How many city-score audit records are in the passage?''
\par\endgroup
%As common in NIAH evaluations, we use Paul Graham essays as the haystack text \citep{kamradt2023needle}. \YZ{Cite Graham essays, check the literature a bit, present a 1k-token example in the appendix?} 
A complete 1k-token passage example is provided in App.~\ref{app:behavioral-1k-example}. We evaluate two types of models (or modes). A Non-thinking model typically emits a final-answer count such as ``Total: 8'', while a Thinking model generates a CoT trace (delimited by \texttt{<think>} and \texttt{</think>} tags in Qwen) before the final-answer count. \footnote{In newer models such as Qwen3 and Gemma-4, one checkpoint supports both Non-thinking and Thinking modes with an on/off switch.} We call records in the prompt \emph{needles} and their generated mentions in the thinking trace \emph{trace items}.

\begin{figure}[htb]
    \centering
    \includegraphics[trim=0 6bp 0 10bp,clip,width=\linewidth,keepaspectratio]{figures/main_figure_v4.pdf}
    \caption{%\textbf{Mechanism and representation comparison of two modes.}
    \textbf{Two retrieval mechanisms and contrasting representations.}
    \textbf{A.} Non-thinking distributes final-query attention across prompt needles. \textbf{B.} Thinking targets successive needles as its trace progresses. Marker $k$ denotes the query before trace item $k+1$. \textbf{C.} PCA projections of states at prompt-needle endpoints (Non-thinking) and trace-item endpoints (Thinking), colored by running index, with numbered centroids. Held-out nearest-centroid classification (NCC) accuracy after whitened 16-component PCA is 46\% for Non-thinking and 98\% for Thinking. Attention and representations are based on Qwen3-8B with 10k-token inputs.\protect\footnotemark See details in Sec.~\ref{app:figure-details}.
    }
    \label{fig:main}
\end{figure}
Current mechanistic understanding is limited for long-context inference and CoT reasoning. First, established analysis in in-context learning and steering often works for short contexts \citep{hendel2023context,todd2024function,turner2024steering,rimsky2024steering}, yet models become brittle in long contexts \citep{liu2024lost}. 
Second, in contrast to static single-token output scenarios, CoT amounts to a \textit{dynamic} procedure: starting from an input prompt $s_{1:t}$, a model emits tokens $s_{t+1},s_{t+2},\ldots$ one by one, which iteratively grows the context $s_{1:t} \to s_{1:(t+1)} \to s_{1:(t+2)} \to \cdots$. 
\footnotetext{%
    An interactive 3D visualization is available at
    \url{https://anonymous.4open.science/r/count-state-geometry-supplement-3B2F/index.html}.
    Click ``JS off'' to enable interaction or download and open it locally.%
}

%To address these difficulties, we study long-context counting, which requires retrieving and aggregating all relevant records without omissions or double counting, letting us examine how retrieval interacts with representations of counting progress during CoT reasoning.
To address these difficulties, we study \textit{long-context counting}, which requires retrieving all relevant records without omissions or double counting, and aggregating needles into a final count. This task serves as an informative testbed, providing a lens for understanding context management in modern LLMs: beyond token-level analysis, we can examine how retrieval interacts with representations of counting progress during CoT reasoning.
Roughly speaking, representations at prompt-needle and trace-item positions follow a curve as the running index increases\footnote{We exclude self-reflection in CoT traces, as detailed in Sec.~\ref{app:native-prompts}.}.
%follow an empirical formula: for certain curve $\boldsymbol{\gamma}: [0,+\infty) \to \R^d$, $\vh_t \in \R^d$ evolves as
%\begin{equation*}
%    \vh_t = \boldsymbol{\gamma}(C(s_{1:t})) + \text{noise}, \qquad \text{where}~C(s_{1:t})~\text{is the needle count of prefix}~s_{1:t}.
%\end{equation*} 
%\LS{This equation is a little bit strange.}
%Here, $C$ counts the prompt needles for Non-thinking modes, and the trace items in the reasoning trace for Thinking modes.\footnote{We exclude self-reflection in CoT traces, as detailed in Sec.~\ref{app:native-prompts}.}
%To better understand this formula, we ask the following questions. 
We call internal counting representations \emph{counter states}, and use \emph{running index} $k$ for the number of prompt needles encountered or trace items enumerated. The \emph{answer state} is the hidden representation at the answer query, labeled by total count $N$. 
%We use \emph{counter state} for an internal representation of counting, \emph{running index} \(k\) for the number of prompt needles encountered or trace items enumerated so far. And at the answer query, we call the hidden representation the \emph{answer state} and labeled by the total count $N$. 
For deeper understanding, we ask: 
%the following questions.
\textbf{Q1} (internal mechanism): what attention mechanisms do the two modes use for retrieving needles? \textbf{Q2} (representation geometry): how compact are representations at needle tokens?  \textbf{Q3} (counter-state evolution): do evolving counter states causally guide subsequent retrieval and final count prediction? 

Overall, our key finding is that two distinct mechanisms exist. Non-thinking models depend on \textbf{broad retrieval}: they broadly attend to all prompt needles at the answer token but produce noisy representations and unreliable counts. Thinking models depend on \textbf{targeted retrieval}: enumeration traces couple successive record retrievals to compact, separable representations of progress, which may help avoid omissions and double counting, thereby improving the count accuracy.
Fig.~\ref{fig:main} illustrates both modes; see~Sec.~\ref{app:figure-details} for details. Below, we summarize our main contributions.

\textbf{1. A comprehensive comparison across model families.} %Across needle counts, prompt length, and model families, 
    %Across model families and scales,
    We characterize how counting accuracy varies with needle count and context length, and show that Thinking substantially improves accuracy.\\
\textbf{2. A mechanistic contrast between the two modes.} We answer Q1 and Q2 by showing that Non-thinking models collect noisy representations at prompt needles %at lower layers 
    through broad retrieval, while Thinking models develop compact representations through targeted retrieval. For Q3, causal intervention results support evolving counter states in CoT traces (Secs.~\ref{sec:non-thinking}--\ref{sec:thinking}).\\
\textbf{3. A controlled experiment on the emergence of two mechanisms.} 
    We train small transformers from scratch under autoregressive losses, with or without CoT traces, which 
    %controls either broad retrieval emerges or targeted retrieval emerges. (Sec.~\ref{sec:emergence}。)
    reproduce key aspects of Thinking and Non-thinking mechanisms (Sec.~\ref{sec:emergence}). 

==> sections/limitations_v1.tex <==
\section{Limitations and Future Work}

We additionally expand our experiments to other relevant tasks like retrieval of the $k$th record and counting within a specified category, see some analyses about behavioral comparisons and retrieval heads interventions in Appendix~\ref{app:additional-task}.

We also use structured enumeration instructions---with indexed and bullet lists---in Non-thinking mode as a controlled comparison in Qwen and Gemma. These experiments support targeted retrieval, counter-state-dependent continuation, and trace-based answer readout under prescribed output formats (Appendix~\ref{app:enumeration}).

\todo{Talk about our limitations and probable future work, including counting is a relative easy tasks, and no ``+1'' circuit. Also, we only prove there's a way, but maybe not the only way.}

==> sections/related_v1.tex <==
\section{Related work}

%\todo{Please help to collect papers and complete this part...}
\paragraph{Counting and long-context retrieval tasks.} 

\TY{(Draft) As LLM-based agents carry out extended workflows, they face accumulated observations and tool outputs, making the ability to retrieve from long histories essential to their decisions \citep{rajasekaran2025context}. The widely used needle-in-a-haystack (NIAH) test isolates this retrieval challenge in a minimal setting: recovering a relevant fact embedded in a long distractor passage \citep{kamradt2023needle}. Moving beyond single-fact retrieval, \citet{hsieh2024ruler,bai2024longbench,song2025countingstars} broaden evaluation to multiple needles, counting, and multi-evidence aggregation, revealing difficulties as context length and task complexity increase. Together with position-sensitive failures such as lost-in-the-middle \citep{liu2024lost}, tshese results highlight the gap between accommodating long inputs and reliably using their contents. 
Thus, we further investigate this question through sparse-record counting which requires accounting for every target occurrence under a clean setting.
 }
 
\YZ{Mention long-context / NIAH tasks. Detail the differences from RULER, etc. Briefly mention the challenges such as lost-in-the-middle. Foundation of frontier capabilities, e.g., agent/harness}
\LS{Explain the difference with regular NIAH tasks, and explain the reasons.}

\paragraph{CoT reasoning analysis.}
\TY{(Draft) Scratchpads and CoT prompting demonstrate the benefits of intermediate computation \citep{nye2021scratchpads}, and theoretical analyses distinguish the additional expressive power supplied by autoregressive intermediate steps \citep{feng2023towards,merrill2024expressive} from learnability under intermediate-sequence supervision \citep{malach2024autoregressive}.
To probe the underlying computation, mechanistic studies trace CoT's effects on information flow and neuron activation \citep{yang2026howcot}, while synthetic arithmetic analyses identify addition circuits operating on helical number representations \citep{kantamneni2025trigonometry}. 
%We further investigate how enumeration interacts with latent count/progress states during long-context inference.
}

\YZ{briefly mention theory papers (many learning theory and TCS papers I think), and briefly mention papers on synthetic arithmetic tasks.}
\YZ{Mention explicit vs implicit reasoning, scattered mechanistic analysis of CoT.}

%\paragraph{Mechanistic evidence standards.}

\paragraph{Counting geometry and state-tracking mechanism.} 
\TY{(Draft) Anthropic's linebreaking study offers a geometric account of counting, identifying low-dimensional curved manifolds encoding character counts \citep{gurnee2025when}. In explicit counting tasks, \citet{hasani2026countscope} identify transferable latent counters through causal interventions.%, but primarily study item sequences and visual arrays rather than CoT-guided long-context retrieval. 
Focusing instead on counting failures, \citet{fu2024letters} link letter-counting errors to repetition and counting complexity without identifying internal causal mechanisms. More generally, controlled studies of predictive belief states \citep{shai2024belief} and finite-state CoT mechanisms \citep{zhang2025fsa} suggest that hidden states compactly summarize task-relevant history. This state-tracking perspective motivates our analysis of how count states evolve and guide retrieval.}

\YZ{Mention Anthropic's manifold, circle / curved representation.} \YZ{Detail the two most relevant papers on counting and state their limitations.}
\YZ{Check whether there is heuristics about state-tracking mechanism (models internally compress context into sufficient state and evolve representations)}


==> sections/related_v2.tex <==
\section{Related work}\label{sec:related}

Connecting the literature on long-context retrieval, CoT reasoning, and counting geometry, our work offers a mechanistic account of how LLMs represent counting geometry, and how they evolve count states in CoT reasoning in realist settings.


\paragraph{Long-context retrieval.} 
NIAH tasks isolate long-context retrieval pressure in a minimal setting: recovering a relevant fact embedded in a long distractor passage \citep{kamradt2023needle}. Moving beyond single-fact retrieval, \citet{hsieh2024ruler,bai2024longbench,song2025countingstars} broaden evaluation to multiple needles, counting, and multi-evidence aggregation, revealing difficulties as context length increases. While \citet{} identified retrieval heads as specialized attention heads, they do not explain long-context failures such as Lost-in-the-Middle \citep{}. In contrast, we present a signal-vs-noise perspective of internal representations, explaining the fallibility of long-context counting in Non-thinking models.


\paragraph{CoT reasoning analysis.} Despite theoretical benefits of CoT reasoning \citep{feng2023towards,merrill2024expressive, malach2024autoregressive}, the actual mechanism of CoT reasoning remains largely unsettled. Unlike static output generation in non-reasoning models, reasoning models generate a sequence of tokens and grow the context dynamically. Recent CoT reasoning analysis focuses on information flow using a range of synthetic tasks \cite{yang2026howcot, kantamneni2025trigonometry} \YZ{cite Fuxin's paper on CoT faithfulness}, but the realistic relevance is unclear. Here, we use long-context counting as a realistic testbed to understand the mechanism of CoT reasoning.

\paragraph{Counting geometry and state-tracking mechanism.} Existing mechanistic work on representation geometry identifies low-dimensional curved manifolds that encode counts \citep{gurnee2025when, engels2025nonlinear,kantamneni2025trigonometry, hasani2026countscope}. The last paper establishes internal counter as a count-encoding mechanism using causal intervention, but its study is limited to simple prompts and non-reasoning models. More broadly, \citet{} find that models use state-tracking mechanism to maintain predictive belief-state, which explains in-context learning \cite{shai2024belief} \YZ{cite Hao Yan's work on task vector, and perhaps a different belief state paper}. In CoT state-tracking tasks, \citet{zhang2025fsa} identify neuron-level mechanisms and measure state compression and distinction. Moving beyond these synthetic tasks, our work confirms that LLMs maintains and iteratively updates count-state in a long-context reasoning task.



